Self-Supervised Point Cloud Completion via Inpainting

When navigating in urban environments, many of the objects that need to be tracked and avoided are heavily occluded. Planning and tracking using these partial scans can be challenging. The aim of this work is to learn to complete these partial point clouds, giving us a full understanding of the object's geometry using only partial observations. Previous methods achieve this with the help of complete, ground-truth annotations of the target objects, which are available only for simulated datasets. However, such ground truth is unavailable for real-world LiDAR data. In this work, we present a self-supervised point cloud completion algorithm, PointPnCNet, which is trained only on partial scans without assuming access to complete, ground-truth annotations. Our method achieves this via inpainting. We remove a portion of the input data and train the network to complete the missing region. As it is difficult to determine which regions were occluded in the initial cloud and which were synthetically removed, our network learns to complete the full cloud, including the missing regions in the initial partial cloud. We show that our method outperforms previous unsupervised and weakly-supervised methods on both the synthetic dataset, ShapeNet, and real-world LiDAR dataset, Semantic KITTI.

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/images/ablation_vis.tex <==
\begin{figure*}[t]
 	\centering
 	\includegraphics[width=0.8\textwidth]{images/Ablations_Figure_renamed.pdf}
 	\vspace{-1em}
 	\caption{Qualitative results for ablation study on ShapeNet and KITTI. Without inpainting, local loss, global loss, and multi-view loss, the network yields noisy output.}
 	\label{fig:ablation_results}
  	\vspace{-18pt}
\end{figure*}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/images/main_results_shapenet.tex <==
\begin{figure*}[t]
 	\centering
 	\includegraphics[width=0.7\textwidth]{images/main_results_shapenet_2.pdf}
 	\vspace{-1em}
 	\caption{Qualitative results on the ShapeNet dataset compared with our baseline, DPC~\cite{insafutdinov2018unsupervised}. Our method is better able to reconstruct fine-grained object details~(back portion of the car and engines on the airplane), produces fewer noisy points for the airplane and produces more uniformly distributed points in the chairs than the baseline.} 
 	\label{fig:qualtitative_results}
 	\vspace{-2em}
\end{figure*} 

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/images/model-diagram.tex <==
\begin{figure*}[t]
 	\centering
 	\includegraphics[trim=0 20 0 0, clip, width=1.0\textwidth]{images/model-diagram-new4.pdf}
 	\vspace{-2em}
 	\caption{\textbf{PointPnCNet Architecture:} Our method first estimates a canonicalized orientation of a partial point cloud, which has some regions missing due to natural occlusions.  We then randomly drop one or more of the regions to create additional synthetic occlusions. We compute global features $e_g$ and local features $P_\ell$ which we combine into an encoding $P$. Our multi-level decoder uses the encoding $P$ to generate a completed point cloud. The global shape loss and local shape loss are only applied to the regions of the output where points are present in the original cloud (before synthetic occlusions) which are shown in \textcolor{red}{red} in $X$, $Y_g$, and $Y_\ell$. The \textcolor{blue}{blue} points in $Y_g$ and $Y_\ell$ are not present in the original cloud, so we have no ground truth about their positions; thus they are not penalized in the loss. The final output of the network is the concatenation of the outputs from $Y_g$ and $Y_\ell$.}
 	\label{fig:model_diagram}
 	\vspace{-1.5em}
\end{figure*} 

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/images/pose_noise_results.tex <==
\begin{figure}[t]
 	\centering
 	\includegraphics[width=0.5\columnwidth]{images/pose_noise_results_line_new2.pdf}
 	\caption{Mean of the Chamfer distance across all ShapeNet categories (Airplane, Car, Chair). Our method is trained with noisy poses, with and without inpainting, shown in \textcolor{green}{green} and \textcolor{red}{red}, respectively. The baseline Gu~\etal~\cite{gu2020weakly} has no added noise.} 
 	\label{fig:pose_noise_results}
 	\vspace{-1em}
\end{figure}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/images/teaser.tex <==
\begin{figure}[t]
\centering
\includegraphics[trim=0 0 0 0, clip, width=0.8\columnwidth]{images/bmvc_fig1.pdf}
\vspace{-1em}
 	\caption{We adopt an \textit{inpainting}-based approach for self-supervised point cloud completion to train our network using only partial point clouds. Given a partial point cloud as input, we randomly remove regions from it and train the network to complete these regions using the input as the pseudo-ground truth. The loss is only applied to the regions which have points in the observed input partial point cloud (\textcolor{red}{red}). Since, the network cannot differentiate between synthetic and natural occlusions, the network predicts a complete point cloud.}
\label{fig:first_page_image}
\vspace{-1.5em}
\end{figure}


% \includegraphics[trim=0 190 0 60, clip, width=0.9\columnwidth]{images/teaser_horizontal_corrected.pdf}

% We adopt an \textit{inpainting}-based approach for self-supervised point cloud completion that allows us to train our network using only partial point clouds. Given a partial point cloud, we randomly remove a region and train the network to complete the entire point cloud from the data itself. Examples (a) and (b) show our approach on a car and a truck.

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/latex/0-abstract.tex <==
\begin{abstract}
When navigating in urban environments, many of the objects that need to be tracked and avoided are heavily occluded.  Planning and tracking using these partial scans can be challenging. The aim of this work is to learn to complete these partial point clouds, giving us a full understanding of the object's geometry using only partial observations. Previous methods achieve this with the help of complete, ground-truth annotations of the target objects, which are available only for simulated datasets. However, such ground truth is unavailable for real-world LiDAR data. In this work, we present a self-supervised point cloud completion algorithm, PointPnCNet, which is trained only on partial scans without assuming access to complete, ground-truth annotations. Our method achieves this via inpainting. We remove a portion of the input data and train the network to complete the missing region. As it is difficult to determine which regions were occluded in the initial cloud and which were synthetically removed, our network learns to complete the full cloud, including the missing regions in the initial partial cloud. We show that our method outperforms previous unsupervised and weakly-supervised methods on both the synthetic dataset, ShapeNet, and real-world LiDAR dataset, Semantic KITTI.
\end{abstract}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/latex/1-intro.tex <==
\input{images/teaser}

\vspace{-1.5em}
\section{Introduction}
\vspace{-0.5em}

%Real world 3D data captured by the scanning devices and depth cameras
%%%%%%%%%%% NEW %%%%%%%%%
Autonomous vehicles often understand the world around them using depth sensors such as LiDAR. However, the LiDAR point clouds are often incomplete even when recorded from multiple viewpoints over time.
%%%%%%%%%%% OLD %%%%%%%%%%
% Autonomous vehicles often understand the world around them using depth sensors such as LiDAR. However, the LiDAR point clouds are often incomplete, since they are recorded from a single viewpoint. 
%%%%%%%%%%%%%%%%
%For an autonomous vehicle, 
%These partial point clouds can greatly reduce the accuracy of tracking and scene flow estimation algorithms \brian{Find citations for this}.
To accurately track objects and plan routes to avoid collisions, it is important for autonomous vehicles to understand the complete shape of surrounding objects.
 %it is crucial to know the complete shape of nearby objects for better navigation, tracking objects, and scene flow estimation. 

%Recent works [cite] often focus on learning a global shape prior of an object and are inefficient in leveraging the local information present in the point cloud data as the network is prone to overfitting based on the structure and position of points in the partial point cloud. In other words, in a LiDAR scene, although the global shape of the objects can be different, there exists a local similarity among the object which can be utilized and learned as a prior for efficient completion of point clouds. 

%%%%%%% NEW
Previous methods~\cite{yuan2018pcn, tchapmi2019topnet, wang2020cascaded, xie2020grnet, wen2020point} have learned to complete partial point clouds but they strongly rely on the availability of ground truth complete shapes as supervision. Since complete point clouds are costly to obtain for real-world scenarios, these methods typically train only from simulated data where ground-truth completions are available. This limitation motivates our approach to learn only from partial point clouds to complete shapes without ever observing the ground-truth completed point clouds during training.


%%%%%%% OLD
% Previous methods~\cite{yuan2018pcn, tchapmi2019topnet, wang2020cascaded, xie2020grnet, wen2020point} have learned to complete partial point clouds using corresponding ground truth complete shape annotations for each partial point cloud as supervision. However, these methods rely strongly on the availability of complete point clouds, which are often costly to obtain for real-world data; these methods typically train only from simulated data where ground-truth completions are available. This limitation motivates our approach to shape completion, which learns only from partial point clouds, without ever observing the ground-truth completed point clouds during training.

%%%%%%%%%

% There are approaches~\cite{gu2020weakly, insafutdinov2018unsupervised} that alleviate the need for ground truth data and perform point cloud completion without the ground truth annotations. However, these methods employ a single encoder and decoder to generate the missing regions in the input partial point cloud. Since the encoder/decoder operate on the entire point cloud as a single resolution, this restricts them to learn only the global shape prior of the point cloud data. Given that point clouds are relatively less structured than images, the global shape of the point cloud data can exhibit a high enough variance based on the structure and position of points in space. This can make these method prone to overfitting on an unseen set of point clouds.

% Although the global shape can vary significantly, there exists similarities among the different point cloud objects of a given category at a more local level and lower resolution. These similarities in the local regions of the point clouds can be utilized and learned as a set of local shape priors to reduce overfitting and complete point clouds more efficiently. 

% This motivates us to propose a method that focuses on learning these local shape priors in parallel to the global shape prior. We propose a novel architecture, PointPnCNet, that employs multiple encoders and decoders operating at different resolutions, to learn this combination of local and global shape priors. 

%%%%%%%%%%% NEW %%%%%%%%%
To this end, our method leverages self-supervision via an inpainting-based approach where we randomly remove regions from the partial point clouds and train the network to complete the entire point cloud. Across multiple training examples, different regions will be occluded and varying regions will be synthetically removed. Because the network does not know which regions were artificially removed and which were naturally occluded in each original partial point cloud, the network learns to attempt to complete the entire point cloud. 

In contrast to images, where a mask can specify the region to inpaint~\cite{liu2020rethinking, pathakCVPR16context, yu2018generative, yeh2017semantic, hong2019deep}, the unstructured nature of point clouds makes it challenging to define which regions the network needs to inpaint. We solve this using a region-aware loss which penalizes only the regions where the original point cloud was present. Additionally, we partition the point cloud into local regions using intersecting half-spaces and encode/decode them separately. This allows the network to learn data-driven embeddings separately for each local region that specialize in individual region-level object parts.  We also encode/decode at the global point cloud level to further allow the network focus on each region jointly with each other. Previous works \cite{insafutdinov2018unsupervised, gu2020weakly} depend on aligning multiple viewpoints of an object during training which can be sensitive to pose alignment errors. While we also incorporate a multi-viewpoint loss, we show that our use of inpainting allows our method to be robust to alignment errors. 

The key contributions of this paper are as follows:  1).  We present a novel inpainting-based self-supervised algorithm that learns to complete missing local regions in an incomplete point cloud without the need for ground truth point cloud completions, 2).  Our multi-level encoder-decoder based architecture, PointPnCNet, partitions the point clouds to learn local and global embeddings to obtain improved completion performance, 3).Our approach outperforms existing methods for unsupervised point cloud completion~\cite{insafutdinov2018unsupervised, gu2020weakly} when evaluated on the standard completion benchmarks of ShapeNet~\cite{chang2015shapenet} and SemanticKITTI~~\cite{behley2019semantickitti}. 

%%%%%%%%%%%% OLD %%%%%%%%%%%
% In the absence of complete point clouds as ground truth, our method leverages the partial point clouds in a self-supervised manner to learn point cloud completion. Our self-supervised algorithm uses an inpainting-based approach where we randomly remove regions from the partial point clouds and train the network to complete the entire point cloud. We apply a loss only to the regions where points were present in the original partial point cloud; we do not apply a loss for the regions that were missing in the original partial cloud, since we do not have any ground-truth information about what the completion in those regions should look like. Additionally, we partition the point cloud into regions using intersecting half-spaces and encode/decode them separately so that the network learns a data-driven embedding for each local region. This embedding allows our network to specialize in individual region-level object parts. Across multiple training examples, different regions will be occluded and varying regions will be synthetically removed. Because the network does not know which regions were artificially removed and which were missing in each original partial point cloud, the network learns to attempt to complete the entire point cloud. 
%%%%%%%%%%%%%%%%
 
 %Thus, the network minimizes the loss by learning to complete the entire point cloud.


% while still being supervised in regions where information in input is present. Additionally, we also partition the point cloud into regions using intersecting half-spaces and encode/decode them separately so that the network learns a data-driven embedding for each local region (termed as \textit{local shape prior}). This local shape prior allows our network to specialize to individual region-level object parts, while still requiring each part to produce a consistent whole. 
% Moreover, the randomness in the region removal minimizes the association between missing and available regions and inhibits the network's ability to decide which regions are missing. As a result, the network ends up maximizing its performance on the task by completion all the regions and hence, the entire point cloud coherently. Therefore, through a combination of random region removal-based inpainting and specialized local shape priors, the network is able to complete real world LiDAR scans, trained only from partial point clouds.

% \brian{I am not sure the below paragraph really describes our method well.} \himangi{I have commented it.}

% Additionally, we partition the point cloud into local regions and encode/decode them separately so that the network learns a data-driven embedding for each local region (termed as \textit{local shape prior}). The local shape prior specializes in generating a certain region of the full point cloud. Although the shape priors of different regions can independently generate a full point clouds in a piece-meal fashion, the priors are generic and operate independent of each other resulting in generation of segments that are not consistent with each other (\eg front of car A generated with back of car B). By conditioning the generation of missing regions based on the available ones, inpainting induces dependency between the priors allowing for a more coherent shape completion. Moreover, the randomness of region removal minimizes the association between missing and available regions and inhibits the network's ability to decide which regions are missing. As a result, the network ends up maximizing its performance on the task by completion all the regions and hence, the entire point cloud coherently. Therefore, through a combination of random region removal-based inpainting and specialized local shape priors, the network is able to complete real world LiDAR scans, trained only from partial point clouds. 

%\brian{This looks like related work. Not sure it belongs here.} \himangi{I mentioned this small paragraph to emphasize the novelty of our method over other methods. I feel it can make the Introduction stronger which is usually the first section read by people.}

%%%%%%%% OLD %%%%%%%%
% In contrast to images, where a mask can specify the region to inpaint~\cite{liu2020rethinking, pathakCVPR16context, yu2018generative, yeh2017semantic, hong2019deep}, the unstructured nature of point clouds
% makes it difficult to define which regions the network needs to inpaint, and the problem of point cloud completion challenging.  We solve this using a region-aware loss which penalizes only the regions where the original point cloud was present. We similarly find it advantageous to use encoders and decoders at local and global levels in our network architecture to allow our network to focus on each region separately. Previous works \cite{insafutdinov2018unsupervised, gu2020weakly} depend on aligning multiple viewpoints of an object during training which can be sensitive to pose alignment errors. While we also incorporate a multi-viewpoint loss, we show that our use of inpainting allows our method to be robust to alignment errors.  
%%%%%%%%%%%%%

%  As a result, our method outperforms previous methods on self-supervised point cloud completion, when evaluated on the standard completion benchmarks of ShapeNet~\cite{chang2015shapenet} and SemanticKITTI~\cite{behley2019semantickitti}.
 
 %Our method uses inpainting which can learn from similar viewpoints as well, making our method more robust to the real-world scenarios. Using the inpainting approach, we show that we can 

% The key insight of our work is that we can learn point cloud completion by randomly dropping regions of the input point cloud and training the network  to inpaint the removed region. This learned inpainting allows our network to complete real world LiDAR scans, trained only from partial point clouds. 

% Using existing methods~\cite{yuan2018iterative}, we canonicalize the input point clouds so that the different point clouds are locally consistent. This prior work does not require the ground-truth pose for training.  This canonicalization allows our approach to learn a robust set of local shape priors that capture local similarities across different point clouds. 
% %Compared to the global structure of an unseen point cloud, there is a higher likelihood of matching the local structures to the learned local shape priors. 
% This in turn allows our method to reduce the generalization gap with respect to unseen point clouds and complete point clouds more efficiently. It further allows to leverage the point cloud data more efficiently and through our experiments, we show that our approach is able to outperform existing methods while also reducing the amount of supervision required in terms of number of partial views per object

%Additionally, previous methods ~\cite{yuan2018pcn, tchapmi2019topnet, wang2020cascaded, xie2020grnet, wen2020point} also use corresponding ground truth complete shape annotations for each partial point cloud as supervision which is costly to obtain in synthetic and real-world data. 
%We believe that for a point cloud completion algorithm to be able to function on real-world LiDAR scans, it should be able to work in the absence of ground truth data. There are approaches\cite{gu2020weakly, insafutdinov2018unsupervised} that alleviate the need for ground truth data and perform point cloud completion without the ground truth complete annotation. However, since they rely on only global shape prior, they are more prone to overfitting and are unable to leverage the local regions of the different point cloud. This motivates us to focus on learning a local shape prior as well as global shape prior by leveraging the data itself through a self-supervised inpainting based approach. By focusing on the local similarities, we are able to reduce the generalization gap since there is a higher likelihood of finding same local shape priors in the test data which in turn reduces the overfitting of a model. By doing so, we are able to reduce the amount of supervision even in terms of number of partial views.




% Recent works address this issue by generating a complete shape to fill the missing regions of a partial point cloud~\cite{yuan2018pcn, tchapmi2019topnet, wang2020cascaded, xie2020grnet, wen2020point}. However, these methods often use direct supervision, requiring a corresponding ground truth complete shape for each partial point cloud. While these annotations are easy to produce for synthetic data, they cannot be easily obtained for data captured in the wild. %Due to the lack of of this complete ground truth shapes in real LiDAR data, 
% To alleviate this restriction, we propose a self-supervised method for point cloud completion. %By training self-supervised point cloud completion in the real world, 
%\brian{Mention improvements cause by training on real data} 

% For our network to learn a local shape prior in a self-supervised manner, we adopt an inpainting-based method, where we randomly drop a region from a partial point cloud and make the network complete the artificially dropped region. By doing so, the network is able to learn a local shape prior of a particular region. Since the location of the region remains consistent across the different objects, our network is able to complete smaller regions and in turn, learns the ability to complete the entire partial scan.



% Since our method does not require ground truth annotations, it is able to work in the wild and leverages the information from the data itself. We highlight this idea by implementing our method on the Semantic KITTI dataset.


% The key contributions of this paper are as follows: 
% \begin{enumerate}
%     \item We present a novel inpainting-based self-supervised algorithm that learns to complete missing local regions in an incomplete point cloud without the need for ground truth point cloud completions.
%     \item Our multi-scale encoder-decoder based architecture, PointPnCNet, partitions the point clouds to learn a combination of local and global embeddings to obtain improved completion performance.
%     %better generalize to unseen point clouds.
%     \item Our approach outperforms existing methods for self-supervised point cloud completion~\cite{gu2020weakly, insafutdinov2018unsupervised} when evaluated on the standard completion benchmarks of ShapeNet~\cite{chang2015shapenet} and SemanticKITTI~\cite{behley2019semantickitti}.
% \end{enumerate}





==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/latex/2-related.tex <==


\vspace{-1.25em}
\section{Related Work}
\vspace{-0.5em}

%%%%%%%%%% NEW
% \textbf{Supervised Point Cloud Completion} Most of the existing 3D shape completion methods~\cite{yuan2018pcn, tchapmi2019topnet, wang2020cascaded, xie2020grnet, wen2020point, wang2020softpoolnet, huang2020pf} use complete ground-truth shape labels and commonly use an encoder-decoder style architecture~\cite{yuan2018pcn,liu2020morphing,xie2020grnet,wang2020point}.  Tchapmi \etal~\cite{tchapmi2019topnet} proposed to generate a point cloud using a hierarchical rooted tree structure. Our architecture builds on the encoder-decoder style of previous work~\cite{yuan2018pcn}. In contrast to the above supervised methods, our proposed approach does not require ground truth annotations and can be trained on LiDAR data, as opposed to the previous methods which are trained only with simulated data.
%%%%%%%%%%


%%%%%%%%%% OLD
\textbf{Supervised Point Cloud Completion} Most of the existing 3D shape completion methods~\cite{yuan2018pcn, tchapmi2019topnet, wang2020cascaded, xie2020grnet, wen2020point, wang2020softpoolnet, huang2020pf} make use of complete ground-truth shape labels. A common approach for point cloud completion is to use an encoder-decoder style architecture~\cite{yuan2018pcn,liu2020morphing,xie2020grnet,wang2020point}. On the other hand, Tchapmi \etal~\cite{tchapmi2019topnet} proposed to generate a point cloud using a hierarchical rooted tree structure. Our architecture builds on the typical encoder-decoder style of previous work~\cite{yuan2018pcn}. In contrast to the above supervised methods, our proposed approach does not require ground truth annotations. This allows our method to be trained using LiDAR data in the wild, as opposed to the previous methods which are trained only with simulated data.
%%%%%%%%%%

\textbf{Weakly-Supervised Methods}
Recently, Gu~\etal~\cite{gu2020weakly} proposed a weakly-supervised approach for point cloud completion where the pose of the input partial point cloud and 3D canonical shape are jointly optimized. Their method is weakly-supervised via multi-view consistency among the multiple partial observations of the same instance. Our method also uses partial point clouds, however, using our inpainting-based approach, our method is able to learn a more accurate completion and is robust to view alignment errors. Other methods also learn 3D shape reconstruction using weak supervision~\cite{yan2016perspective, zhu2017rethinking, tulsiani2018multi}. Among these, Differentiable Point Clouds~(DPC)~\cite{insafutdinov2018unsupervised} jointly predicts camera poses and a 3D shape representation given two image views of the same instance. The geometric consistency between the estimated 3D shape and the input images is enforced using an end-to-end differentiable point cloud projection.  We show in the results that we significantly outperform this method.

%This method, unlike ours, requires color information.

%Other methods such as Perspective Transformer Networks~\cite{yan2016perspective} also rely on different 2d views of a 3d object and use pre-computed geometric transformation to generate a single 3d shape. In comparison to these methods, we operate fully in the 3D point cloud space, allowing us to process data that do not map well to projective transforms.%with complex scan patterns.

\textbf{Image Inpainting}
In the area of image inpainting~\cite{liu2020rethinking, pathakCVPR16context, yu2018generative, yeh2017semantic, hong2019deep, zhan2020self}, Zhan \etal~\cite{zhan2020self} proposed self-supervised partial completion networks (PCNets) to complete an occluded object's mask and content in the input image. Our method takes inspiration from Zhan \etal~\cite{zhan2020self} for shape completion in 3D point clouds. %\himangi{
However, due to the structured nature of images, often a mask can be used to specify the region to inpaint. In 3D point clouds, where the data is unstructured and sparse in nature, it is difficult to specify a ``mask" for the regions to inpaint. There is ambiguity between regions that have been ``masked out" and regions that are naturally occluded, making the task of inpainting challenging for point cloud data.
%}
%removed and specify such a mask which makes the task of inpainting challenging.}

%\himangi{
\textbf{Point Cloud Inpainting} Some of the previous methods~\cite{fu2018point, yu2020point, fu20203d, zhao2020pui, chen2020point, hu2019local} have also explored inpainting in the point cloud domain. However, these methods either use ground truth during training~\cite{yu2020point, zhao2020pui}, rely on template-matching within a data sample~\cite{fu2018point, fu20203d, hu2019local}, or project a point cloud into 2D structured representation~\cite{chen2020point}. Our method is novel in the sense that it uses inpainting directly on the point clouds without any ground truth information while leveraging large datasets to learn domain-specific priors. % learns a prior over entire training data.
%}







==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/latex/3-methods.tex <==
\vspace{-1.25em}
\section{Method}
\vspace{-0.5em}
%\subsection{Problem Definition}

The point cloud completion problem can be defined as follows: given an incomplete set of sparse 3D points $X$, sampled from a partial view of an underlying dense object geometry $G$, the goal is to predict a new set of points $Y$, which mimics a uniform sampling of $G$. 
% In practice, $X$ is usually obtained from a partial view of $G$ at a single viewpoint.



% \subsection{Canonical Pose Estimation}
% \label{sec:preprocessing}

% \himangi{For our method, we do not assume ground truth poses. To canonicalize our data, we use two different approaches. For ShapeNet~\cite{chang2015shapenet} data, we use IT-Net~\cite{yuan2018iterative} to generate pose predictions for each object. Specifically, we use the classification branch of the IT-net to generate the pose transformations, as it does not require the ground-truth pose annotations for training. For autonomous driving data (e.g. for Semantic KITTI~\cite{behley2019semantickitti}) we use an object detector to generate oriented bounding boxes which give us an orientation to canonicalize the partial point clouds. With the consistency in the canonicalized partial point clouds, the network is better able to generalize across partially occluded samples with different regions missing. Additionally, we do not assume that the partial point clouds will be perfectly aligned after the canonicalization. In the Results section, we analyse the alignment between the canonicalized partial point clouds and emphasize that our method is robust to noisy alignment.}
\input{images/model-diagram}
\vspace{-1em}
\subsection{Self-supervised Inpainting}
\label{sec:inpainting}
\vspace{-0.5em}
%%%%%%%%%% NEW
In our self-supervised inpainting-based approach to learn to complete full point clouds using only partial point clouds, we randomly remove regions of points from a given partial point cloud and train the network to inpaint these synthetically removed regions. The original partial point cloud is then used as a pseudo-ground truth to supervise the completion. Since we do not have the complete ground-truth point cloud, supervision is only applied to the regions of the original point cloud that contain points (i.e. unoccluded regions). 
%%%%%%%%% OLD
% To enable our model to learn full point cloud completion using only partial point clouds, we adopt a self-supervised inpainting-based approach. At training time, we randomly remove regions of points from a given partial point cloud and train the network to inpaint these synthetically removed regions. The original partial point cloud is then used as a pseudo-ground truth to supervise the completion. Since we do not have the complete ground-truth point cloud, supervision is only applied to the regions of the original point cloud that contain points (i.e. unoccluded regions). 
%%%%%%%%%%

%, avoiding the local minima of predicting the one-to-one mapping between an input partial point cloud and its corresponding partial point cloud generated after removing a region. The network ends up completing the entire point cloud since it will be the full approximation of all possible mappings.

%In addition to inpainting, we also use partitioning of the point cloud for the network to learn a local shape prior.
%%%%%%%%%%%%% NEW
% Specifically, given a partial point cloud, we estimate its canonical frame using a learned method~(Sec.~\ref{sec:experiments}) and transform it to obtain a canonicalized partial point cloud $X$. We show that our method is robust to errors in this canonicalization~(Sec.~\ref{sec:robustness}).  We then partition the canonicalized partial point cloud into $N$ regions and remove points of any particular region with probability $p$. This results in a synthetically occluded cloud $\hat{X}$ that we use for training.
%%%%%%%%%%% OLD
% Specifically, given a partial point cloud, we estimate its canonical frame using a learned method~(Sec.~\ref{sec:experiments}) and transform the point cloud to obtain a canonicalized partial point cloud $X$. We show that our method is robust to errors in this canonicalization~(Sec.~\ref{sec:robustness}).  We then partition the canonicalized partial point cloud into $N$ regions. For each region, the points contained within that region are removed, with probability $p$, which results in a synthetically occluded cloud $\hat{X}$ that can be used to train our method. 
%%%%%%%%%%%%%%

% \brian{This seems out of place here.} \himangi{The below paragraphs will be helpful in explaining how inpainting is able to complete the point cloud. In addition to the randomness, the network also learns a local shape prior to complete the regions. This section can be used to give the intuition as to how the completion is actually happening by writing about what each encoder and decoder is doing. We can maybe rename the subsection to mention that the following section explains the intuition of completion, so that the below paragraphs do not feel out of place.}

% \dave{This paragraph seems to be out of place, lacks context, and will be confusing to the reader.}
% We use multiple encoders and decoders for completion. 
% % With the help of one-hot encoding, each decoder specializes in completing a certain region, allowing it to learn a shape prior localized to that region. This local shape prior helps in generating a localized region-level point cloud segment of the entire point cloud. 
% With the help of one-hot encoding, each decoder specializes in completing a certain region, allowing it to learn a shape prior and generate a point cloud segment localized to that region.
% % In our method, we also canonicalize the partial point clouds before passing it as input to our shape completion network. 
% The network leverages the consistency across the canonicalized partial point clouds to learn a set of local shape priors that can generalize across partially occluded samples with different missing regions. By pooling the information of available regions across samples, the local shape priors allow the decoder to generate all the regions for an input partial point cloud, hence creating the full point cloud. Moreover, conditioning the inpainting on the available point cloud regions lead to a more object-specific completion.

% With the consistency across the canonicalized partial point clouds, the network is able to learn a local shape prior and generalize across partially occluded samples with different missing regions. 
% The inpainting task creates an association among the local shape priors, allowing the missing regions to be generated in the context of the entire object. 
% However, the prior can be very generic and may not be enough for an object-specific completion. 
% Here, the randomness in the region removal and inpainting of that region allows the network to learn the representation of that object and makes the process of generation to happen at a more object-specific manner. Moreover, the stochastic nature of region removal avoids the network to learn a one-to-one mapping between an input partial point cloud and its corresponding partial point cloud generated after removing a region.  The network therefore ends up completing the entire point cloud since it will be the best approximation of all possible mappings.

%%%%%%%%% NEW %%%%%%%%
The network leverages the information of available regions across samples and embeds each region separately that can generalize across partially occluded samples with different missing regions. Further, due to the stochastic nature of region removal, the network cannot easily differentiate between the synthetic and original occlusions of the input partial point cloud, making the network learn to complete the point cloud. Thus, the combination of inpainting, random-region removal, and region-specific embeddings enables the model to generate all the regions and create a complete point cloud.
%%%%%%%%%%% OLD
% The network leverages the information of available regions across samples and learns embeddings of individual parts of an object that can generalize across partially occluded samples with different missing regions. Additionally, due to the stochastic nature of region removal, the network cannot easily differentiate between the synthetic and original occlusions of the input partial point cloud $\hat{X}$. With the combination of random-region removal, inpainting, and learned embeddings, the network learns to generate all the regions and creates a complete point cloud.
%%%%%%%%%%%%%%%

%\dave{This is an over-claim}
%, as it covers the combination of all possible synthetic occlusions and all possible initial partial point clouds that could produce the given input cloud.




%\dave{This is unrelated}
%In parallel to the local branches, we also have a global branch that provides an overall shape context at a higher resolution and helps in a more consistent generation across all the regions. 
% The combination of randomness in region removal, inpainting, and local shape prior gives the network the ability to fill the missing regions and predict a complete point cloud. 



% Our method is self-supervised, as we rely only on training data comprised of partial point clouds and do not require the supervision of complete ground truth point clouds. Because the input is only a partial point cloud (observed from only a single viewpoint with self-occlusions) and not the full point cloud, it cannot be treated as a full ground-truth of the point cloud completion. We address this issue in Section~\ref{sec:losses}.

%Specifically, we subdivide the partial cloud into fixed regions . 



% \begin{algorithm}[t]
% \label{algo:offline}
% \caption{PointPnCNet}
% \end{algorithm}

\vspace{-1em}
\subsection{Network Architecture}
\vspace{-0.5em}

Figure~\ref{fig:model_diagram} depicts the architecture and training flow of our network, Point Cloud Partition-and-Completion Network (PointPnCNet). We use a multi-level encoder-decoder architecture to allow the network to focus on different parts of an object. We present the evaluations of various alternate designs of our method in the appendix.
%}
%We encode and decode the separate regions using parallel encoder-decoder streams, with shared weights.
\vspace{-0.5em}
\subsubsection{Multi-Level Encoder}
\label{sec:multi-scale-encoder}
\vspace{-0.5em}
%%%%%%%%%%% NEW
 Our encoder consists of multiple, parallel encoder streams that encode the input partial point cloud at global and local levels. The global-level encoder operates on the full-scope of the object while a local-level encoder focuses on a particular region of the object. Since a local encoder only sees points in a given local region and is invariant to other parts of the shape which may be missing, local encoders make the network robust to occlusions by focusing on individual object parts separately. Global encoder further enhances shape consistency by focusing on regions jointly with each other.
%%%%%%%%%% OLD
%  Our encoder consists of multiple, parallel encoder streams that encode the input partial point cloud at the global and local levels. Using local encoders has two advantages: first, it allows the network to focus on the individual parts of the object.  Second, the local encoder only sees the points in a given local region and thus is invariant to the other parts of the object that may be missing.  This allows our network to be robust to different types of occlusions.
 %%%%%%%%%%%%%%%
 Given a partial point cloud, we estimate its canonical frame using a learned method~(Sec.~\ref{sec:experiments}) and transform it to obtain a canonicalized partial point cloud $X$. We show that our method is robust to errors in this canonicalization~(Sec.~\ref{sec:robustness}).  
 We then partition the canonicalized partial point cloud using intersecting half-spaces that are produced by the coordinate planes after canonicalization. This effectively separates the space into eight 3D octants as shown in Figure~\ref{fig:model_diagram}. While other types of partitioning could be used, we found this subdivision to be simple and reasonably effective. Rather than a strict partitioning, we allow a small overlap between neighboring regions such that points in the overlap are present in both regions. This helps to avoid seams at boundaries.
Let $X_{i}$ consist of the points in the region $i$. After partitioning, we remove points of any particular region with a probability $p$ to simulate a synthetic occlusion. We use this synthetically occluded point cloud $\hat{X}$ as input to our inpainting network.
 %%%%%%%%%%%% OLD %%%%%%%%%%%
%  Specifically, given a partial point cloud, we estimate its canonical frame using a learned method~(Sec.~\ref{sec:experiments}) and transform it to obtain a canonicalized partial point cloud $X$. We show that our method is robust to errors in this canonicalization~(Sec.~\ref{sec:robustness}).  We then partition the canonicalized partial point cloud into $N$ regions and remove points of any particular region with probability $p$. This results in a synthetically occluded cloud $\hat{X}$ that we use for training.
 
%  To create the local encodings, we divide the point cloud space into local regions; let $X_{i}$ consist of the points in the region $i$.  In our experiments, we use the intersecting half-spaces produced by the coordinate planes, after estimating the canonical orientation of each object.  This effectively separates the space into eight 3D octants as shown in Figure~\ref{fig:model_diagram}.
 %%%%%%%%%%%%%%%%%%%%%%%%
% We randomly remove points in each of these regions~(octants) and then train the network to inpaint the missing points. 

%%%%%%%%%%%% OLD %%%%%%%%%%%
% While other types of partitioning could be used, we found this subdivision to be simple and reasonably effective. Rather than imposing a strict partitioning in the point cloud space, we allow a small overlap between neighboring regions to avoid seams at boundaries. The points in these boundary regions are considered to be in both regions.
 %%%%%%%%%%%%%%%%%%%%%%%%

% After partitioning the original partial input point cloud into a set of local regions, some of these regions are randomly removed for inpainting~(Sec~\ref{sec:inpainting}). The remaining regions are aggregated together and fed as input to the global encoder, $E_{g}$, to give an embedding $e_g$ (Figure ~\ref{fig:model_diagram}). 

%%%%%%%%%%%% OLD %%%%%%%%%%%
% Once the original partial point cloud $X$ is partitioned into a set of local regions, some of these regions are randomly removed, to simulate a synthetic occlusion.  We use this synthetically occluded point cloud $\hat{X}$ as input to our inpainting network. The points in the remaining regions are aggregated together and passed as input to the global encoder, $E_{g}$, to give a global embedding $e_g$ (Figure ~\ref{fig:model_diagram}). 
%%%%%%%%%%%%%%%%%%%%%%%%

% As described in the previous section, the original partial input point cloud is partitioned into a set of local regions based on an imposed structure. Some of these regions are randomly removed to train the network to inpaint them as part of the output. After the random region removal process, the remaining regions are aggregated together and input to the global encoder, $E_{g}$ to give an embedding $e_g$ (as shown in Figure~\ref{fig:model_diagram}). 


%This allows the local encoder to isolate smaller scale features, unique to each region. \dave{We already explained why we need local encoders at the top of this section.}
%The local embeddings are subjected to a feature dropout where the embeddings of the dropped regions are removed (the same regions removed for the global encoder). 
%\dave{Just say that we only input the regions that have not been dropped out to the local encoder} 


% In parallel, all the regions obtained from the original partial input point cloud are input separately to a set of $N$ local encoders, $E^1_{\ell},\ldots, E^N_{\ell}$ as per their location in the imposed structure. In our case, we use $N=8$ regions, structured in a grid, as described above. The set of learned parameters are shared by each of these $N$ local encoders. The output from each of these encoders is subjected to a similar region dropout described above, where the encodings of the dropped regions are removed. %some of the outputs are randomly set to zero so as to emulate the random region removal for self-supervised completion. 
% The network architecture of the encoders is similar to PCN~\cite{yuan2018pcn}.

% In a similar manner, we can optionally define a finer-grained $3 \times 3 \times 3$ grid and a set of corresponding encoders. We can partition the point cloud based on this grid and input the different regions of the point cloud to the respective encoders for this $3 \times 3 \times 3$ grid. This process can be repeated any number of times based on the computational budget and point cloud resolution. When having multiple grids, we can randomly choose both the number as well as the resolution of regions to \textit{drop} in the input to $E_{1\times 1 \times 1}$.

%\subsubsection{Multi-Resolution Feature Aggregation}
%%%%%%% NEW
The points in the remaining regions are aggregated together and passed as input to the global encoder, $E_{g}$, to give a global embedding $e_g$~(Figure~\ref{fig:model_diagram}). 
In parallel, each remaining region $X_{i}$ is separately encoded by a local encoder, $E_{\ell}$ to obtain a local embedding for that region, $e^{i}_{\ell}$. To aggregate the local feature embeddings, each embedding $e^{i}_{\ell}$ is fed as input into an attention module, consisting of an MLP layer, that generates a set of weights $w_{i} = \phi (e^{i}_\ell)$. These weights are used to weigh each of the embeddings $e^{i}_{\ell}$ in a linear combination to form the aggregate embedding $P_\ell = \sum_{i} \mathbbm{1}_i w_{i} \, e^{i}_\ell$, where $\mathbbm{1}_i$ is an indicator function which equals 1 if region $i$ is present~(i.e. present in the original partial point cloud $X$ and not randomly removed) and 0 otherwise.  
% We consider a region to be present in the original partial point cloud if the number of points in that region exceeds a defined threshold. 
We then perform a channel-wise max-pooling across the global encoding $e_g$ and the attention-weighted local encoding $P_\ell$, as $P = \max (e_g, P_\ell)$.
%%%%%%%%%% OLD %%%%%%%%%%%%%
% In parallel, each remaining region $X_{i}$ is also separately encoded by a local encoder, $E_{\ell}$ to obtain a local embedding for that region, $e^{i}_{\ell}$. To aggregate the local feature embeddings, each embedding $e^{i}_{\ell}$, corresponding to the output of the local encoder $E_{\ell}$ for the points in region $X_{i}$, is input into an attention module.  The attention module consists of an MLP layer which generates a set of weights $w_{i} = \phi (e^{i}_\ell)$. These weights are used to weigh each of the embeddings $e^{i}_{\ell}$ in a linear combination to form the aggregate embedding $P_\ell = \sum_{i} \mathbbm{1}_i w_{i} \, e^{i}_\ell$, where $\mathbbm{1}_i$ is an indicator function which equals 1 if region $i$ is present (i.e. present in the original partial point cloud $X$ and not dropped out) and zero otherwise.  We consider a region to be present in the original partial point cloud if the number of points in that region exceeds a defined threshold. We then perform a channel-wise max-pooling across the global encoding $e_g$ and the attention-weighted local encoding $P_\ell$, as $P = \max (e_g, P_\ell)$.
%%%%%%%%%%%

%from $E^1_{\ell},\ldots, E^N_{\ell}$.


% Once we obtain the feature embeddings of the remaining regions, $e^{i}_{\ell}$, corresponding to the output of encoders $E^1_{\ell},\ldots, E^N_{\ell}$, the embeddings are combined using a feature aggregation module. 

% This weighted encoding represents a more fine-grained local-level information that enables the network to understand the shape of the point cloud and provide better generation of missing regions. 
% The information present in this encoding provides the network an opportunity to fill in the gaps in the information present in the encoding coming from the $E_{1\times 1 \times 1}$ encoder. 


\vspace{-0.5em}
\subsubsection{Multi-Level Decoder}
\vspace{-0.5em}
Our decoder consists of multiple decoder streams that work in parallel to decode the fused embedding $P$ (Figure~\ref{fig:model_diagram}). The global decoder $D_{g}$ takes the embedding $P$ as input and attempts to generate an entire completed point cloud $Y_g$.
%generates a point cloud with inpainted missing regions corresponding to the original input point cloud. 
% Our decoder consists of multiple decoder streams that work in parallel to decode the fused embedding. As shown in the Figure~\ref{fig:model_diagram}, the decoder $D_{g}$ takes the fused embedding as input and generates a point cloud with inpainted missing regions corresponding to the original input point cloud. The structure of this decoder is similar to the decoder in PCN~\cite{yuan2018pcn}.
In parallel, we use a local decoder $D_{\ell}$ to decode the points in each region of the input space. The embedding $P$ is concatenated with a one-hot vector indicating each region's location and create a region-specific embedding. Through one-hot encoding, each decoder specializes in completing a certain region and learns a region-specific embedding. The decoder takes as input these region-specific embeddings and generates a subset of the output point cloud localized to the respective region $Y_\ell^i$. The generated local regions are combined together to obtain the full point cloud $Y_\ell$.
%Each of these decoded regions uses this embedding as input and generates a subset of the output point cloud corresponding to their respective region. %location in the grid. 
%The set of learned parameters are shared by each of these 8 decoders.  
The multi-level output generated by the network captures the details of the object at global and local levels. The outputs of the multi-level decoder streams, $D_{\ell}$ and  $D_{g}$, are concatenated to form the final prediction of our network as $Y$.

%a hierarchical feature representation of the underlying point cloud data at global and local levels. 


% \begin{figure*}[t]
%  	\centering
%  	\includegraphics[width=1.0\textwidth]{figures/model-diagram.pdf}
%  	\caption{\textbf{PointPnCNet Architecture:} The multi-scale encoder takes canonicalized input partial point cloud and outputs aggregated feature $P$ with features from global and local levels. The multi-scale decoder uses $P$ to generate completed point cloud at global and local levels.}
%  	\label{fig:model_diagram}
% \end{figure*} 

%\subsubsection{Region Removal and Inpainting}
%\subsection{Weighted Chamfer Distance-Based Losses}
\vspace{-1em}
% \input{images/main_results_shapenet}
\subsection{Point Cloud Completion Losses}
\label{sec:losses}
\vspace{-0.5em}
%%%%%%%%%%% NEW %%%%%%%%%
The standard loss used for comparing two point clouds is the Chamfer Distance (CD). It is a bi-directional permutation invariant loss over two point clouds representing the nearest neighbor distance between each point and its closest point in the other cloud. In our method, 
we use an asymmetric Weighted Chamfer Distance loss, $\mathcal{L}_{wcd}$, defined as, 
%%%%%%%%%%% OLD
% The standard loss used for comparing two point clouds is the Chamfer Distance (CD), which is a bi-directional permutation invariant loss over two point clouds representing the nearest neighbor distance between each point and its closest point in the other cloud. In our method, 
% we use an asymmetric Weighted Chamfer Distance loss $\mathcal{L}_{wcd}$, 
%%%%%%%%%%%%%%%%%%%%
% \begin{equation}
% \footnotesize
% \mathcal{L}_{wcd} (\mathcal{X}, \mathcal{Y}) = \frac{(1 - \beta)}{|\mathcal{X}|}\sum_{x \in \mathcal{X}} \min_{y \in \mathcal{Y}}\|x - y\|_2  +  
%     \frac{\beta}{|\mathcal{Y}|}\sum_{y \in \mathcal{Y}} \min_{x \in \mathcal{X}} \|y - x\|_2
% \label{equ:cd_global_loss}
% \end{equation}
\begin{equation}
\footnotesize
\mathcal{L}_{wcd} (X, Y) = \frac{(1 - \beta)}{|X|}\sum_{x \in X} \min_{y \in Y}\|x - y\|_2  +  
    \frac{\beta}{|Y|}\sum_{y \in Y} \min_{x \in X} \|y - x\|_2
\label{equ:cd_global_loss}
\end{equation}
% \begin{equation}
% \footnotesize
% \begin{split}
%     \mathcal{L}_{wcd} (\mathcal{X}, \mathcal{Y}) &= (1 - \beta)\cdot\frac{1}{|\mathcal{X}|}\sum_{x \in \mathcal{X}} \min_{y \in \mathcal{Y}}\|x - y||_2 \\
%     & + \beta\cdot
%     \frac{1}{|\mathcal{Y}|}\sum_{y \in \mathcal{Y}} \min_{x \in \mathcal{X}} \|y - x||_2
% \end{split}
% \label{equ:cd_global_loss}
% \end{equation}

%$\mathcal{L}_{\ell}^i = \mathbmm{1}_i \mathcal{L}_{wcd} (S_i, Y^i_\ell)$ where $\mathbmm{1}_i$ is an indicator function which equals 1 if region $i$ is present in the original partial point cloud $X$ and zero otherwise.
%%%%%%%%%%%% NEW %%%%%%%%%
\noindent where $X$ is the original partial point cloud used here as pseudo-ground truth and $Y$ is the output. 
Importantly, we only compute the loss for the regions that are present in $X$. A weight of $(1-\beta)$ is applied to the first term in Eqn.~\ref{equ:cd_global_loss} which penalizes the distance from each point in $X$ to its nearest neighbor in $Y$. This term enforces that the output point cloud $Y$ should contain points that are close to those in $X$. Note that the input to the network is $\hat{X}$, which has synthetic occlusions, not $X$, which is the original partial point cloud. A weight of $\beta$ is applied to the second term in Eqn.~\ref{equ:cd_global_loss} to penalize the distance from each point in $Y$ to its nearest neighbor in $X$. 
We do not expect this term to reach 0 for a well-trained network since $X$ only contains a partial point cloud, while output $Y$ contains the entire point cloud; we still find it a helpful regularization. 
We impose the following variants of $\mathcal{L}_{wcd}$ on the model,
%%%%%%%%%%%%% OLD %%%%%%%%%%%%
% \noindent where $X$ is the original partial point cloud and $Y$ is the output. 
% Importantly, we only compute the loss for the regions that are present in the original partial point cloud $X$. A weight of $(1-\beta)$ is applied to the first term in Eqn.~\ref{equ:cd_global_loss} which penalizes the distance from each point in $X$ to its nearest neighbor in $Y$. This term enforces that the output point cloud $Y$ should contain points that are close to those in the original partial point cloud $X$. Note that the input to the network is $\hat{X}$, which has synthetic occlusions, not $X$, which is the original partial point cloud. A weight of $\beta$ is applied to the second term in Eqn.~\ref{equ:cd_global_loss} to penalize the distance from each point in $Y$ to its nearest neighbor in $X$. 
% %\himangi{Need to write the next lines in more detail, explain why the loss can go to zero, and how we are avoiding it}
% We do not expect this term to reach 0 for a well-trained network since $X$ only contains a partial point cloud of the object, whereas $Y$ is trained to output the entire point cloud; still, we find that it is a helpful regularization.
%%%%%%%%%%

% A higher weight, $(1 - \beta)$, is applied to the first term in Equation~\ref{equ:cd_global_loss} which penalizes the distance from each point in $\mathcal{X}$ to its nearest neighbor in $\mathcal{Y}$. This enforces that the output point cloud should contain points that are close to those in the input. 

% A lower weight $\beta$ is applied to the second term which penalizes the distance from each point in $\mathcal{Y}$ to its nearest neighbor in $\mathcal{X}$. This term is not expected to reach 0 for a well-trained network since the input $\mathcal{X}$ only contains a partial point cloud of the object, whereas $\mathcal{Y}$ is trained to output the entire point cloud. 

%\himangi{
%A trivial solution to our proposed loss function does not exist. 
% To clarify, $X$ is not the input to the neural network. For a partial point cloud $X$, we apply a random synthetic occlusion to create a further reduced point cloud $\hat{X}$ which is input to the network.
%Thus if the network outputs $\hat{\mathcal{X}}$, it will not minimize the loss; the loss will only be minimized if the network infers missing parts of the point cloud and outputs $\mathcal{X}$, which is a partial point cloud \emph{before} the synthetic occlusion.
%}
%%%%%%%%%% NEW v2 %%%%%%
% \textbf{Inpainting-Global Loss:} This loss focuses on the overall object shape. We impose it as the Weighted Chamfer Distance (Eqn.~\ref{equ:cd_global_loss}) between $X$ and the output of the global decoder $Y_{g}$ and define it as $\mathcal{L}_{wcd} (X, Y_{g})$. 
%%%%%%%%% NEW %%%%%%
\textbf{Inpainting-Global Loss:} This loss acts as a \textit{global shape loss}, focusing on the overall shape of an object. We impose it as the Weighted Chamfer Distance (Eqn.~\ref{equ:cd_global_loss}) between original partial point cloud $X$ and output of the global decoder $Y_{g}$ and define it as $\mathcal{L}_{wcd} (X, Y_{g})$. 
%%%%%%%%%%% OLD %%%%%%%%%%
% \textbf{Inpainting-Global Loss:} 
% % \himangi{Write the importance of global loss} 
% We use the Weighted Chamfer Distance (Eqn.~\ref{equ:cd_global_loss}) to estimate the distance between the original partial point cloud $X$ and the output of the global decoder $Y_{g}$ and define it as $\mathcal{L}_{wcd} (X, Y_{g})$. This loss reasons about the overall shape of an object.
%%%%%%%%%%%%%%

% The first term above calculates the average distance between the predicted point cloud $Y_{g}^{out}$ and its nearest neighbor in the input partial point cloud $\mathcal{X}$.  

% The Chamfer distance is appropriate when the full ground-truth completed point cloud is available.  

%This loss reweights the distances from our generated cloud and the distances from the points in the target cloud as a function of the weighting parameter $\beta$.  




% However, because $\mathcal{X}$ is only a partial point cloud, there might not be a point in $\mathcal{X}$ that corresponds to each point in the predicted point cloud $\mathcal{Y}$.


% This calculates the average nearest neighbor point distance between the predicted point cloud $\mathcal{X}$ and the input partial point cloud $\mathcal{Y}$. A higher weight is used for the Chamfer distance applied from input partial point cloud to predicted shape making the predicted point cloud cover the input partial point cloud efficiently. On the other hand, a higher weight to the Chamfer distance from predicted point cloud to input partial point cloud often makes the points collapse to a certain region of the input partial point cloud.

%Distance to our generated cloud, $S_g$, is minimized as more points are brought closer to the ``ground truth" surface, but does not insentience covering the more of the object. Distance to $S_\ell$, however incentives more coverage of the target surface, but can pull points away from near surfaces.
% As $\beta$ is increased, more the loss incentives more accurate generated points, but decreases the loss associated with poor coverage of the complete model. In this work, we find \brian{???} produces a good balance of accuracy and coverage.
%This calculates the average nearest neighbor point distance between the predicted point cloud $\mathcal{S}_{g}$ and ground truth point cloud $\mathcal{S}_{\ell}$. Here, $\beta$ defines the weight for each distance. We give more weight to the Chamfer distance applied from ground truth to predicted shape. This forces the predicted point cloud to cover the ground truth point cloud. On the other hand, giving more weight to the Chamfer distance from predicted point cloud to ground truth point cloud often makes the points collapse to a certain region of the input partial point cloud.

%\subsubsection{Local Shape Loss}
% The standard method of supervising completion using the Chamfer loss is to apply this loss over the full generated and target point cloud, which we refer to as  \textit{global shape loss}. While this loss has the benefit of capturing the full space of the target shape, it has some drawbacks when it comes to our self-supervised method.
% Since we are only using partial point clouds in our pipeline, we need to handle the local regions of our input definitely, as some may be empty due to synthetic occlusion, for which we have completion data, while others were occluded in the original sensor capture. For this later class of region, we have no completion information, but we do not want penalize our network for attempting to complete this regions. 

%Since we have encoder-decoder streams operating at different resolutions and regions of the point cloud, 

% Our target point cloud in Equation~\ref{equ:cd_loss} is the partial input point cloud generated from a particular viewpoint of a given object.  

% Thus, there will be correlations in which regions of space are missing due to self-occlusions.

% For the network to learn to complete the entire point cloud, we apply the above Weighted Chamfer Distance in two ways - in a \textit{global shape loss} and in a \textit{local shape loss}. 

% \textbf{Global Shape loss: }
% For the global shape loss, we apply the weighted CD between the output of the decoder $D_{g}$ and the input partial point cloud. 

%With the multiple views present for a given instance, we apply the weighted CD between the output of the decoder $D_{g}$ with all the partial point cloud views of the instance as multiple ground truths.
%%%%%%%%%%%% NEW 3 %%%%%%%%%%
% \textbf{Inpainting-Local Loss:} We impose this loss as the Weighted Chamfer distance between each region output $Y_\ell^i$ from local decoder $D_{\ell}$ and corresponding partitioned region $X_i$ in $X$ where $i$ indexes over regions. While Inpainting-Global loss considers the entire $X$ to find the nearest neighbor, Inpainting-Local loss differs in that it only considers the partitioned region $X_i$ to find the nearest neighbor. Thus, it acts as a \textit{local shape loss} that enables the network to learn region-specific shapes and embeddings and focus on the finer details of an object. We do not penalize regions that are missing in $X$ where a region is considered missing if the number of points in that region is below a certain threshold. Inpainting-Local Loss is therefore defined as, $\sum_{i}\mathbbm{1}_i \cdot \mathcal{L}_{wcd} (X_{i}, Y_\ell^i)$ where the indicator function $\mathbbm{1}_i$ equals 1 if region $i$ is present in $X$ and 0 otherwise. 
%%%%%%%%%%%%% NEW 2 %%%%%%%%%%%
\textbf{Inpainting-Local Loss:} We impose Inpainting-Local loss as the Weighted Chamfer distance between each region output $Y_\ell^i$ from local decoder $D_{\ell}$ and corresponding partitioned region $X_i$ in the original partial point cloud $X$ where $i$ indexes over regions. While Inpainting-Global loss considers the entire $X$ to find the nearest neighbor, Inpainting-Local loss differs in that it only considers the partitioned region $X_i$ to find the nearest neighbor. Thus, it acts as a \textit{local shape loss} that enables the network to learn region-specific shapes and embeddings and focus on the finer details of an object. We do not penalize regions that are missing in $X$ where a region is considered missing if the number of points in that region is below a certain threshold. The Inpainting-Local Loss is therefore defined as, $\sum_{i}\mathbbm{1}_i \cdot \mathcal{L}_{wcd} (X_{i}, Y_\ell^i)$ where the indicator function $\mathbbm{1}_i$ equals one if region $i$ is present in $X$ and zero otherwise. 
%%%%%%%%%%% NEW %%%%%%%
% \textbf{Inpainting-Local Loss:} This loss acts as a \textit{local shape loss} that enables the network to learn region-specific shapes and embeddings and focus on the finer details of an object. We impose it as the Weighted Chamfer distance between each region output $Y_\ell^i$ from local decoder $D_{\ell}$ and corresponding partitioned region $X_i$ in the original partial point cloud $X$ where $i$ indexes over regions. We do not penalize regions that are missing in $X$ where a region is considered missing if the number of points in that region is below a certain threshold. Thus, the Inpainting-Local Loss is defined as, $\sum_{i}\mathbbm{1}_i \cdot \mathcal{L}_{wcd} (X_{i}, Y_\ell^i)$ where the indicator function $\mathbbm{1}_i$ equals one if region $i$ is present in $X$ and zero otherwise.  
%%%%%%%%%% OLD %%%%%%%%%%%
% \textbf{Inpainting-Local Loss:} \himangi{Write the importance of local loss} We also define a \textit{local shape loss} that is the Weighted Chamfer distance between each region's output from the local decoder $D_{\ell}$ and the corresponding partitioned regions in the original partial point cloud $X$. We do not penalize for regions that are missing in the original partial point cloud, where we define a region to be missing if the number of points in that region is below a certain threshold. Thus, the local shape loss can be written as:  $\sum_{i}\mathbbm{1}_i \cdot \mathcal{L}_{wcd} (X_{i}, Y_\ell^i) $ where $i$ indexes over regions, $X_{i}$ represents the points in each region from the original partial point cloud $X$, $Y_\ell^i$ represents the output from the local decoder $D_{\ell}$ for region $i$, and $\mathbbm{1}_i$ is an indicator function which equals one if region $i$ is present in $X$ and zero otherwise. 
%%%%%%%%%%%%%%%%%%
%\dave{How do you define a present region or missing region?}.
%\himangi{There is a line in this paragraph - we define a region to be missing if the number of points in that region is below a certain threshold - which defines a present region and missing region.}
% In order to handle this, we define a \textit{local shape loss} loss based on the above Weighted Chamfer distance that would allow our network to complete point clouds effectively in both synthetically and naturally occluded regions. 
% We associate the output of our network with each region, $\hat{X}_i$, and apply the weighted Chamfer loss between those points and the points in the associated region. 
% We do not penalize regions where the number of input points in that region is below a certain threshold. \dave{This part is very unclear and I don't understand it at all}

%First we have the \textit{global shape loss} that we apply as the weighted CD between the output of the decoder $D_{1\times 1 \times 1}$ and the ground truth, \ie, input partial point cloud without any regions removed artificially.With multiple views present for a given instance, we apply the weighted CD between the output of the decoder $D_{1\times 1 \times 1}$ with all the partial point cloud views of the instance as multiple ground truths.

%Next we have the \textit{local shape loss} that we apply as the weighted CD between the different region outputs of the decoders $D^2,\ldots, D^2 and the corresponding partitioned regions in the input partial point cloud.

% \input{tables/shapenet_main}

%%%%%%%%%%%%%% NEW %%%%%%%%%%%
\textbf{Multi-View Consistency:} Similar to Gu~\etal~\cite{gu2020weakly}, our method uses multi-view consistency as an auxiliary loss. Their method explicitly performs pose estimation. Similarly, we perform an estimated pose canonicalization (weakly supervised, Sec.~\ref{sec:experimental_setup}). We also show later~(Sec.~\ref{sec:robustness}) that our method is robust to canonicalization errors. During training, we sample a view $k$ from $V$ partial views of an object $X$ given as $X^{1}, \ldots, X^{V}$. Since all the views of an object correspond to the same object, for input partial point cloud $X^{k}$, the loss is computed with all views $X^{1}, \ldots, X^{V}$. We define a global inpainting multi-view consistency loss as $\sum_{j=1}^{V}\mathcal{L}_{wcd} (X^{j}, Y_{g}^{k})$ where $X^{j}$ is the $j^{th}$ view of $X$ and $Y_{g}^{k}$ is the global output from decoder $D_{g}$. We also define local inpainting multi-view consistency loss as $\sum_{i}\sum_{j=1}^{V}\mathbbm{1}^j_i \cdot \mathcal{L}_{wcd} (X^{j}_{i}, Y_\ell^{i,k})$ where $i$ indexes over regions, $X^{j}_{i}$ is the $i^{th}$ region of view $X^j$, 
$Y_\ell^{i,k}$ is the region output from local decoder $D_{\ell}$ for input $X^{k}_{i}$, and $\mathbbm{1}^j_i$ is $1$ if region $i$ is present in $X^{j}$ and $0$ otherwise.
During training, we sum the losses as, $\sum_{j=1}^{V}\mathcal{L}_{wcd} (X^{j}, Y_{g}^{k}) + \sum_{i}\sum_{j=1}^{V}\mathbbm{1}_i \cdot \mathcal{L}_{wcd} (X^{j}_{i}, Y_\ell^{i,k})$. This multi-view information is only available at training time.

%%%%%%%%%%% OLD %%%%%%%%%%%%%%%%%%%
% \textbf{Multi-View Consistency:} Given multiple views of an object, our method leverages this information similar to Gu~\etal~\cite{gu2020weakly}. Similar to their method, which explicitly performs pose estimation, we perform an estimated pose canonicalization (weakly supervised, as explained below); however, we show that our method is robust to canonicalization errors (see Sec.~\ref{sec:robustness}).
% During training, we sample view $k$ from multiple views of an object instance, $X^{1} ... X^{V}$, where $V$ is the number of views. Since all the views of an object correspond to the same object, we consider the completion of $X^{k}$ and compute its loss with respect to all views. We define the global shape multi-view consistency loss as: $\sum_{j=1}^{V}\mathcal{L}_{wcd} (X^{j}, Y_{g}^{k})$,  $X^{j}$ refers to the original partial point cloud of each $j$th view, and $Y_{g}^{k}$ refers to the output from the decoder $D_{g}$ of the sampled view $k$. Similarly, we define the local shape multi-view consistency loss as: $\sum_{i}\sum_{j=1}^{V}\mathbbm{1}_i \cdot \mathcal{L}_{wcd} (X^{j}_{i}, Y_\ell^{i,k})$ where $i$ indexes over regions, $X^{j}_{i}$ represents the region $i$ in the $j$th view, 
% $Y_\ell^{i,k}$ represents the output from the decoder $D_{\ell}$ for the sampled view $k$ in region $i$, and $\mathbbm{1}_i$ is $1$ if region $i$ is present in $X$ and $0$ otherwise.
% % we select one as input and apply synthetic occlusions as described in Section~\ref{sec:inpainting}. We then select a subset of the available views and compute the shape loss for each cloud, independently\dave{which shape loss?  the one from sec 3.5.1 or 3.5.2?  please clarify this in more detail}.
% At training time, we use the sum of the global shape loss and local shape loss: $\sum_{j=1}^{V}\mathcal{L}_{wcd} (X^{j}, Y_{g}^{k}) + \sum_{i}\sum_{j=1}^{V}\mathbbm{1}_i \cdot \mathcal{L}_{wcd} (X^{j}_{i}, Y_\ell^{i,k})$. 
% %\himangi{There can be an assumption that since we have multiple views of the same object which cover all the viewing directions, we can get a full point cloud. However, 
% This multi-view information is only available at training time.%} 
% %Note that the multi-view consistency is an optional part of our method; unlike previous work~\cite{gu2020weakly}, we can learn from even a single viewpoint due to inpainting.  In other words, 
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\paragraph*{Multi-View Consistency vs Inpainting: }\brian{I think this section should be moved to experiments} Previous work~\cite{gu2020weakly} depends on multiple viewpoints to approximate the complete target shape. %obtain a target for the network to complete the missing points.  
%On the other hand, our approach can learn even when the input and target clouds are taken from the same viewpoint via inpainting. Our method generates synthetic occlusions via region dropout, and our network learns to complete these dropped out points. Learning from the same, or similar, views is especially helpful when we cannot easily obtain observations of an object from all viewing angles; for example, in real world autonomous driving datasets, objects are usually only viewed from a small range of viewpoints.


%Further, all the multiple views may not be correctly aligned with each other, even after our canonical pose estimation or the pose prediction step of prior work~\cite{gu2020weakly}. Methods using multiple views can be sensitive to the pose alignment, whereas, inpainting can also operate on similar viewpoints. In the Results Section, we show an analysis of our method with noisy poses with and without inpainting. Thus, we show that being able to learn from  \emph{inpainting} gives a large boost in the performance compared to previous work. 
%At the same time, adding multiple viewpoints still allows our method to improve performance.

%\dave{More details should be added here - how is this different from previous work; why can't we just merge all of the views and treat that as ground-truth, etc}

%apply the weighted CD between the outputs of the decoders $D^1_{2\times 2 \times 2},\ldots, D^8_{2\times 2 \times 2}$ with the corresponding regions across each of the partial point clouds views of the instance.


%We do not penalize regions that are missing in the input point cloud where a region is defined to be missing if the number of points in that region is below a certain threshold. With multiple views present for a given instance, we apply the weighted CD between the outputs of the decoders $D^1_{2\times 2 \times 2},\ldots, D^8_{2\times 2 \times 2}$ with the corresponding regions across each of the partial point clouds views of the instance.

% \paragraph*{Multi-view Shape Consistency}
%  Since, we have $\mathcal{V}$ number of multiple views, we can have a $\mathcal{V*V}$ loss computed between the predictions and ground truth. In our work, we choose a reference frame out of the multiple views. To maintain the consistency in the shape of the multiple views, we compute the loss between the output of the reference frame with the $\mathcal{V}$ number of views of ground truth point cloud.

% \paragraph*{Multi-view Global Consistency Loss}
% We compute this loss between the output of the global decoder and the input partial point cloud. Since, we do not have the ground truth complete shape, we consider the input partial point cloud as the ground truth itself. This loss will penalize the network over the global shape information. This will push the points to create a global shape and cover the ground truth. $<Write importance of this loss here>$

% \paragraph*{Multi-view Octant Consistency Loss}
% This loss is computed between the multiple views of an octant. Due to the absence of ground truth, we consider the input octant as the ground truth itself. Note that the loss is only computed for the octants that are present in an input partial point cloud and the loss is zeroed out for the octants that are absent. This loss will penalize the network over the local shape information and will force the output points to cover the ground truth points of a part of an object. $<Write importance of this loss here>$

% \paragraph*{Multi-view Combined Output Consistency Loss}
% This loss is computed over the concatenated global and local output which will penalize the network over the entire global and local information altogether. $<Write importance of this loss here>$

% \subsection{Inference}
% During test-time, we use a single view of an object. The multiple views are only available during training. To get the final completed point cloud, we concatenate the output from the different scale decoders $D_g$ and $D_{\ell}$. We do not remove regions at inference time. Otherwise, the network during inference is the same as described above. 



%We apply the same pre-processing as in Sec.~\ref{sec:preprocessing}.
%The point cloud is appropriately aligned to the grid and partitioned to be input to the grid encoders. 
% The feature output from the encoders is subjected to multi-resolution feature aggregation and is then input to the multi-resolution decoders to generate the point cloud at different resolution. We combine the output from the different decoders as the final completed point cloud. 
% Since the grid decoders are aligned to the grid and operate in a specific region in the point cloud space, they are able to localize and learn a well-formed shape prior about specific designated regions and thereby, improve the overall quality of point cloud completion. The encoders and decoders can learn the shape prior from the entire set of point cloud data, and generate the shape of a specific region jointly conditioned on this shape prior and the collective feature information from the other regions of a given point cloud.



==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/latex/4-experiments.tex <==


% \input{tables/shapenet_main}
% \input{tables/kitti_main}
% \input{tables/shapenet_views}
% \input{tables/agg_ablation}

\vspace{-1.5em}
\input{images/main_results_shapenet}
\section{Experiments}
\vspace{-0.5em}

\label{sec:experiments}
\subsection{Implementation Details}
\vspace{-0.5em}
%\textbf{Implementation Details:}
During test-time, we use a single view of an object. The multiple views are only available during training. To get the final completed point cloud, we concatenate the output from multi-level decoders $D_g$ and $D_{\ell}$. We do not remove regions at inference time. Otherwise, the network during inference is the same as described above.
For consistency with prior work~\cite{gu2020weakly}, we resample each partial point cloud $X$ to have a total of 3096 points.
% For regions that are not considered missing, we resample each region to have 387 points, such that the total number of points over all the regions is 3096 (387 points $\times$ 8 regions).
% For all encoder and decoder blocks of PointPnCNet, we use the architecture from PCN~\cite{yuan2018pcn}. 
PointPnCNet uses architecture from PCN~\cite{yuan2018pcn} for encoder and decoder blocks. The model is trained from scratch for 400K iterations with batch size of 32, learning rate of 5e-4 decayed by 0.5 after every 100K iterations and $\beta = 0.25$ in $\mathcal{L}_{wcd}$. Please refer to appendix for more details.

% %%%%%%%%%% OLD %%%%%%%%%%%%%
% During test-time, we use a single view of an object. The multiple views are only available during training. To get the final completed point cloud, we concatenate the output from the different scale decoders $D_g$ and $D_{\ell}$. We do not remove regions at inference time. Otherwise, the network during inference is the same as described above.

% For consistency with prior work~\cite{gu2020weakly}, we resample each partial point cloud $X$ to have 3096 points. Any region with less than a minimum threshold of points~(details in the appendix) is considered missing \himangi{Should I indicate the threshold here? And its reason in the appendix?} and is not used when computing the Inpainting-Local loss. For regions that are not considered missing, we resample the points within each region to 387 points, such that the total number of points over all the regions is 3096 (387 points * 8 regions).  %is the entire partial point cloud without any partitioning. For t
% %%%%%%%%%%%%%%%%%%%

%with reference to the center of an axis-aligned bounding box estimated via IT-Net\cite{yuan2018iterative}, we divide the input point cloud into 8 parts~(octants). 

%$\mu$ at 4. %For the regions with number of points less than $\nu$, it is considered to be absent and is replaced with $128$ zeros as points. 
%Since the input point cloud is partial and has less number of points, setting a high threshold would yield more absent octants. For octants that are present, we resample the number of points available to an upper bound of $387$ points such that the total number of points over all octants is $3096$, the same as for the high resolution encoder.


% We restrict the number of points in each active region to a fixed number, $387$, downsampling regions that exceed this size and resampling points in regions with less than this number of points. This ensures that each region has equal weight in the final loss and that the total number of points used by the high and low resolution encoders are equivalent.
%To avoid a strict division of the input point cloud, we introduce an overlap parameter in the boundaries such that the octant boundaries overlap with each other by some percentage. 


%In the absence of actual complete ground truth point cloud in our self-supervised inpainting-based approach, the input being given to PointPnCNet is subjected to random region removal and the ground truth corresponding to the point cloud generated by PointPnCNet is the original input partial point cloud. For the high-resolution encoder and corresponding \textit{global shape loss}, the size of the ground truth is fixed at 8192 points. For the lower resolution encoders and corresponding textit{local shape loss}, the size of the ground truth per octant is fixed at 512 points.

%The architecture of the encoders and decoders in PointPnCNet are similar to that 
%%%%%%%%%%% OLD %%%%%%%%%
% We use the encoder and decoder architecture as described in PCN~\cite{yuan2018pcn} in all the encoder and decoder blocks of PointPnCNet. The network is trained from a random initialization with a batch size of 32 and a learning rate of 5e-4, decayed by a step of 0.5 after every 100K iterations. For computing the loss, we use $\beta = 0.25$.
%%%%%%%%%%%%%%%
%For the weighted Chamfer Distance loss, we set $\beta$ as 0.25. %The above details are the same for both synthetic and real-world datasets.
% division into parts 1, 2, 3; size of octants
% e1, e2, e3; architecture details
% fuzzy boundary
% train from scratch;
% dropout; architecture details
% decoders; architecture details
% batch size; learning rate; iterations; learning rate decay

\vspace{-1em}
\subsection{Experimental Setup}
\vspace{-0.5em}
\label{sec:experimental_setup}
Following the evaluation protocol of Gu~\etal~\cite{gu2020weakly}, we test our approach on ShapeNet~\cite{chang2015shapenet} and Semantic KITTI~\cite{behley2019semantickitti}. ShapeNet has ground truth annotations for each object class which allows us to evaluate how well our method generates completed shape. On the other hand, Semantic KITTI allows us to evaluate the robustness of our method on real LiDAR data. 

The observations are transformed to a canonical frame (a shared reference frame which aligns all instances of a class) using canonical frame predictions generated via IT-Net~\cite{yuan2018iterative} for ShapeNet and predicted bounding boxes obtained from OpenPCDet~\cite{openpcdet2020} for Semantic KITTI. We use IT-Net for ShapeNet as it is trained in a weakly-supervised manner from only classification labels and learns to align the instances of each class, without any pose supervision. In general, any pose estimator can be used here. We evaluate the robustness of our method to this canonical frame estimation in Sec.~\ref{sec:robustness}.

% We evaluate the importance of each component in our approach through an exhaustive ablation study.

%This section describes our experiment setup in terms of datasets used for evaluation, preprocessing steps, metrics and implementation details. This is followed by the description of the different experiment we conduct, their results and our observations. We train a separate network for each object category which is able to generalize to different objects in the same category.

%%%%%%%%%% NEW %%%%%%%%%%%
\textbf{ShapeNet:} ShapeNet~\cite{chang2015shapenet} is a synthetic dataset with 3D CAD models. We report our results on three categories, airplanes, cars, and chairs, that are commonly used in the related works~\cite{insafutdinov2018unsupervised, gu2020weakly}.  We use the same data split provided by DPC~\cite{insafutdinov2018unsupervised},  where RGB-D data is generated for random camera views with fixed translation, similar to Gu \etal~\cite{gu2020weakly}. For evaluation, we use ground truth point clouds provided by DPC~\cite{insafutdinov2018unsupervised} which are densely sampled from ShapeNet meshes and downsampled to 8192 points.

\textbf{Semantic KITTI:} We evaluate our method for a real-world scenario using KITTI~\cite{behley2019semantickitti}. Previous methods~\cite{xie2020grnet, gu2020weakly, wen2020point, yuan2018pcn} have a standard protocol of evaluation on real-world data by testing on the cars of KITTI only. We adopt the same protocol in our work. Following Gu \etal~\cite{gu2020weakly}, we train over the parked car instances~(which have multiple views captured when a LiDAR sensor moves through the scene and scans a parked car from different locations) with sequences 00 to 10 (excluding 08) as train set and sequence 08 as test set. The train set consists of 507 parked car instances and 46152 observations, while the test set has 229 parked car instances and 16296 observations. 



% Please refer to appendix for more details. 


%%%%%%%%%%%%%%%%%%%%%

% \subsection{Datasets}
%%%%%%%%%%% OLD %%%%%%%%%%%%
% \textbf{ShapeNet:} ShapeNet~\cite{chang2015shapenet} is a synthetic dataset with available 3D CAD models. We report our results on three categories commonly used in the related works~\cite{insafutdinov2018unsupervised, gu2020weakly} and having large sets of models: airplanes, cars, and chairs and use the data and splits (70\% train, 10\% validation, 20\% test) provided by DPC~\cite{insafutdinov2018unsupervised},  where RGB-D data is generated for 5 random camera views with fixed translation, similar to Gu \etal~\cite{gu2020weakly}. 
% % We obtain a point cloud from the RGB-D data by backprojecting 2.5D depth images to 3D similar to Gu \etal~\cite{gu2020weakly}. In contrast to DPC~\cite{insafutdinov2018unsupervised}, we do not use the color information. 
% For evaluation, we use ground truth point clouds provided by DPC~\cite{insafutdinov2018unsupervised} which are generated by dense sampling of points from ShapeNet meshes and downsampled to 8192 points. 

% At training time, four views are used in our multi-view consistency loss, while only one view is used during inference time. For both training and inference, we use IT-Net~\cite{yuan2018iterative} to generate canonical frame predictions for each input partial point cloud and transform it to a canonical orientation. The rest of the details about Shapenet are provided in the appendix. \himangi{Mention IT-Net?}
%%%%%%%%%%%%%%%%%%%%%%
% The centers of the oriented clouds are then shifted to the origin before passing it to our shape completion network. Specifically, we use the 3D partial shape classification branch of IT-net pre-trained on ModelNet40 to generate the pose transformations, as it does not require the ground-truth pose annotations for training. Since our method does not require perfect pose alignment, using IT-Net pretrained on ModelNet40 instead of ShapeNet is sufficient for our purpose, as it represents an off-the-shelf canonical frame estimator for our model classes.  We refer the reader to IT-Net~\cite{yuan2018iterative} for details on this pose canonicalization method.

%then recentered to the origin.%, such that their mean lies on the the origin. %We use the transformation which is predicted as an intermediate result by the classification network.
%After canonicalizing the input point cloud, we compute the axis aligned bounding box for the point cloud and shift its center to origin. 

% - how generated - depth images details
% - count of train, val, test of car, chair and plane
% - pretrained model of IT-net used to canonicalize
% - axis aligned bbox to make translation zero

% category wise split for shapenet, number of 3D models used, number of partial point clouds = N*5 (5 views)
% car: train/test/val 5247/1500/750
% airplane: train/test/val 2831/810/404
% chair: train/test/val 4744/1356/677


% \begin{figure*}[t]
%  	\centering
%  	\includegraphics[width=\textwidth]{figures/ablation_vis.pdf}
%  	\caption{Qualitative results of the ablation studies of PointPnCNet. First, second, third, and fourth row shows the results on the test set of car, chair, plane, and Semantic KITTI dataset respectively.}       
%  	\label{fig:ablation_results}
% \end{figure*}

%%%%%%%%%%% OLD
% \textbf{Semantic KITTI:} We evaluate our method in a real-world scenario using the KITTI odometry dataset~\cite{behley2019semantickitti}. 
% % for the analysis of our point cloud completion  method. 
% Following Gu \etal~\cite{gu2020weakly}, we train over the parked car instances with sequences 00 to 10 (excluding 08) as the train set and sequence 08 as the test set. The train set consists of 507 unique car instances and 46152 observations, while the test set has 229 instances of parked cars and 16296 observations. The observations are transformed to a canonical frame using the predicted bounding boxes obtained from OpenPCDet~\cite{openpcdet2020}. The rest of the detail about Semantic KITTI are provided in the appendix. \himangi{Mention OpenPCDet?}
%%%%%%%%%%%%%%%%%

% At training time, we subdivide the observations of a single instance into groups of 20 sequential observations and randomly sample a set of four views for multi-view training. 

% The observations are transformed to a canonical frame using the predicted bounding boxes obtained from OpenPCDet~\cite{openpcdet2020}.
%To prepare the data, we consider a car instance and collect its occurrences in a window of 20 frames. From this window, we randomly sample sets of 4 views. To help our network learn the shape prior, we canonicalize the input using predicted bounding boxes obtained from OpenPCDet []. The ground truth point cloud, needed to evaluate the output of our method, is created by merging the occurences of the car instance in the window of 20 frames.
% When evaluating accuracy on this dataset, all 20 frames are combined using ground truth odometry to form the ground truth shape of each instance. This merged cloud is only used for evaluation and is not present during training. At inference time, only a single view is used.

Although having no complete ground truth information in KITTI creates some limitations in its evaluation, testing on this dataset shows the ability of our method to handle real-world LiDAR data. By combining the evaluations on a real-world dataset~(KITTI) and a synthetic dataset~(ShapeNet), which has ground truth annotations, we are able to present a more thorough evaluation. This is the standard evaluation procedure following Gu \etal~\cite{gu2020weakly}.

% dataset preparation
% size of train and test
% partial GT
% detected boxes

% \subsection{Implementation Details}


% \subsection{Metrics}
\textbf{Metrics:} 
%We adopt the standard metric as used in the previous works \himangi{cite other works too} \cite{gu2020weakly} to quantitatively evaluate the complete shape generated by our method. 
Our primary metric for quantitatively evaluating shape completion is the \textit{Chamfer Distance (CD)}, as is used in previous works~\cite{gu2020weakly,yuan2018pcn,wang2020cascaded}. We define this metric in its weighted form in Equation \ref{equ:cd_global_loss}. For evaluation, to compare with the ground-truth completed point cloud, we equally weight each component with a $\beta$ of $0.5$.  
%It computes the average closest distances between the points of predicted point cloud $\mathcal{S}_{g}$ and ground truth point cloud $\mathcal{S}_{\ell}$. 
Additionally, we follow Gu \etal~\cite{gu2020weakly} and report each component of the Chamfer distance independently: the mean distance from each predicted point to its nearest true point described as \textit{Precision}, and the mean distance from each true point to its nearest predicted point described as \textit{Coverage}. \textit{Precision} describes how well the predicted points match the local shape, while \textit{Coverage} is related to how much of the shape is completed. We also evaluate the Earth Mover's Distance~(EMD)~\cite{yuan2018pcn}, which finds a bijection between the predicted point cloud and the ground truth point cloud that minimizes the average distance between corresponding points. Like previous work, we also evaluate the F-score@1\%~\cite{xie2020grnet}.

%Since there are no complete ground truth point clouds for KITTI, we also evaluate the F-score~\cite{xie2020grnet}, with respect to closest point distance.

%compute two other metrics to estimate the coverage between the two point clouds. The first term of Equation \ref{equ:cd_metric} is called \textit{Precision} which ..... and the second term is called \textit{Coverage} which ......

%\begin{equation}
%\begin{split}
%    \mathcal{CD} {(S_g, S_\ell)} &= \frac{1}{|S_g|}\sum_{x \in \mathcal{S}_{g}} \min_{y \in \mathcal{S}_{\ell}}\|x - y||_2 \\
%    & + \frac{1}{|S_\ell|}\sum_{y \in \mathcal{S}_{\ell}} \min_{x \in \mathcal{S}_{g}}\|y - x||_2
%\end{split}
%\label{equ:cd_metric}
%\end{equation}

% \input{tables/shapenet_pose_noise}
% \brian{Should describe other metrics here too (At least a reference to the specific definition of point cloud EMD and F1 score)} 


% \input{tables/kitti_main}

% \input{tables/shapenet_main}
% \input{tables/table2_3}
\vspace{-1em}
\subsection{Point Cloud Completion Results}
\vspace{-0.5em}
%%%%%%%%%%% NEW %%%%%%%%%%%
We compare with the current state-of-the-art unsupervised methods, DPC~\cite{insafutdinov2018unsupervised} and Gu~\etal~\cite{gu2020weakly}. 
%%%%%%%%%% OLD
% We compare our method to the unsupervised methods DPC~\cite{insafutdinov2018unsupervised} and Gu~\etal~\cite{gu2020weakly}, which represent the state-of-the-art performance.
%%%%%%%%%%%%%
%Table~\ref{table:shapenet_main_results} and Table~\ref{table:kitti_main_results} summarizes the results of the comparison of our method PointPnCNet with existing approaches that do not use ground truth complete point clouds for the task of point cloud completion. 
%%%%%%%%%%%%% NEW %%%%%%%%%
Table~\ref{table:shapenet_main_results} shows our method outperforming the baseline methods on the synthetic ShapeNet dataset, producing lower Chamfer distances across all shape categories. \textit{Precision} and \textit{Coverage} metrics also improve, showing that our method produces more accurate points and better covers the full object shape.
%%%%%%%%%%%% OLD %%%%%%%%%%%%%%%%%%%%
% Table~\ref{table:shapenet_main_results} shows our method outperforming the baseline methods on the synthetic ShapeNet dataset, producing lower mean Chamfer distances across all of the shape categories. Additionally, we see an improvement in the \textit{Precision} and \textit{Coverage} metrics, showing that our method produces more accurate points and better covers the full object shape. 
%%%%%%%%%%%%%%%%%
% We also report the Earth Mover Distance (EMD) metric in Table~\ref{table:emd_shapenet}. Our method is able to outperform the baseline DPC~\cite{insafutdinov2018unsupervised} with respect to this metric. 
%%%%%%%%%% NEW %%%%%%
Our method is also able to outperform DPC~\cite{insafutdinov2018unsupervised} as per the Earth Mover Distance (EMD) metric (Table~\ref{table:kitti_agg_emd}b).
Since the code for \cite{gu2020weakly} is not publicly available, the EMD metric on that method cannot be evaluated.
%%%%%%%%%%%%%%%% OLD %%%%%%%%%
% Our method is also able to outperform the baseline DPC~\cite{insafutdinov2018unsupervised} with respect to the Earth Mover Distance (EMD) metric as shown in Table~\ref{table:emd_shapenet}.
% Since the code of \cite{gu2020weakly} is not publicly available, the EMD metric on that method could not be evaluated.
%%%%%%%%%%%%%%


% not just improves the accuracy of the generated points, , but also the  of the target object. 
%the Airplane, Cars, and Chairs categories of ShapeNet.
%From the table, we can observe that for all the categories of ShapeNet, PointPnCNet is able to outperform the existing methods by achieving a significantly smaller chamfer distance on the test set of point cloud objects. 
%%%%%%%%%%%%% NEW %%%%%%%%%%
We further show in Table~\ref{table:agg_ablation_sem_kitti}a that our method outperforms the previous state-of-the-art~\cite{gu2020weakly} on the Semantic KITTI dataset, generating outputs that are significantly more accurate than~\cite{gu2020weakly}.
%%%%%%%%%%% OLD
% We further show that our method outperforms the previous state-of-the-art weakly supervised result~\cite{gu2020weakly} on the Semantic KITTI dataset, shown in Table~\ref{table:kitti_main_results}, generating significantly more accurate outputs than previous methods~\cite{gu2020weakly}. 
%%%%%%%%%%%%%
% This emphasizes that \emph{inpainting} helps the network to learn from similar viewpoints when capturing data from a moving vehicle. \dave{Agreed with Brian; this is an unsupported statement}
%%%%%%%%%%% NEW %%%%%%%%%%%
The KITTI dataset is more realistic than ShapeNet. With samples having a range of sparsity (since real-world LIDAR gets sparse with distance), it represents the data available in self-driving scenarios. We also show improvement compared to a simple densification baseline (Densified Input in Table~\ref{table:agg_ablation_sem_kitti}a) which suggests that our method is indeed completing the partial point clouds rather than simply densifying them. This densification baseline uniformly samples points within the volume of a local surface that is approximated as an ellipsoid, formed using eigenvalues for 10 nearest neighbors of each point in input partial point cloud. We also conduct a uniformity analysis whose results we report in the appendix.
%%%%%%%%%%%%%%% OLD %%%%%%%%%%%%%
% The KITTI dataset is more realistic than ShapeNet since it represents the data available in self-driving scenarios. %\himangi{
% Additionally, we compare our method to a simple densification baseline~(details in the appendix). The improvement over this baseline in Table~\ref{table:kitti_main_results} shows that our method is completing the partial point clouds instead of simply densifying the partial point cloud. Uniformity metrics are also reported in the appendix.
% %}
%%%%%%%%%%%%%%%

%We can again observe that our method PointPnCNet is able to outperform other methods. In fact, PointPnCNet is able to reduce the Chamfer Distance on Semantic KITTI by more than 50\% compared to existing state-of-the-art method.
%\input{tables/shapenet_views}
\input{tables/shapenet_main}
\input{tables/table2_3}
\input{tables/cd_emd_fig_table}

\vspace{-1.125em}
\subsection{Qualitative Results}
\vspace{-0.5em}
%To provide a further comparison of our approach with existing methods, we visualize some of the point clouds generated by the different methods for the different categories/datasets.

% Figure~\ref{fig:qualtitative_results} depicts the point cloud completions generated by our method for example objects in each of the ShapeNet categories we test over, with completions generated by the unsupervised method, DPC~\cite{insafutdinov2018unsupervised} as comparison. We observe that our method better covers the target object, with a more uniform distribution over the target surface. 
We present the qualitative results of our method for each category of ShapeNet in Figure~\ref{fig:qualtitative_results} and KITTI in Figure~\ref{fig:ablation_results}. In comparison to the baseline DPC~\cite{insafutdinov2018unsupervised}, we observe that our method is able to better cover the target object with a more uniform distribution over the target surface and accurately reconstructs the fine-grained object details. For example, our method is able to complete the back of the car and the side mirror whereas the baseline outputs noisy points. For chairs, our method generates more uniformly distributed points whereas the baseline outputs patches/clusters of points in that location. This highlights the fact that our method is better able to generalize and complete the unseen regions of incomplete shapes.

% It can observed that our method is able to complete the back of the car and the side mirror whereas the baseline outputs noisy points in those locations. For chairs, the generated point cloud by our method is more uniformly distributed whereas the baseline only shows patches/clusters of points in that location. This highlights the fact that our method is better able to generalize and complete the unseen regions of incomplete shapes.


% This is particularly evident in the back of the chair and the body of the airplane, where our method uniformly completes the unseen regions. 
%of our method is less noisy and better distributed in the space. By allowing the features to be capture at different resolutions and by pinning the encoder to localize and learn shape prior for specific regions in the space, our method is able to better position the points in the space such that they provide a more complete point cloud compared to existing methods that rely on a single-resolution based feature representations.
% We compare our self-supervised point cloud completion network with \cite{gu2020weakly} and present the results in Table~\ref{table:shapenet_main}. As can be seen, our method is able to outperform the baseline on Airplane, Cars, and Chairs categories. In the Figure ...

% Similary, in Table~\ref{table:kitti_main_results}, PointPnCNet outperforms the baselines. In the Figure....

% quantitative refering to the tables

% qualitative referring to the visuals


%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\columnwidth]{figures/multi_views_comparison_v2.pdf}
%	\caption{Qualitative results on varying the number of views  given as input to the PointPnCNet. First, second, third, and fourth row shows the results on the test set of car, chair, plane, and Semantic KITTI dataset respectively.}       
%	\label{fig:views_results}
%\end{figure}



\input{images/ablation_vis}
\vspace{-1.125em}
\subsection{Ablation Study}
\vspace{-0.5em}

\noindent \textbf{Inpainting Loss:} Region removal to create synthetic occlusions and the task of inpainting are removed, \textbf{Multi-View Loss:} The multi-view loss is removed from our training method. Each partial point cloud is used to supervise its own, synthetically occluded completion, \textbf{Global Level:} We remove the Inpainting-Global Loss, global encoder $\mathbf{E_g}$ and global decoder $\mathbf{D_g}$ from our completion pipeline. \textbf{Local Level:} The Inpainting-Local loss, local encoder $\mathbf{E_{\ell}}$ and local decoder $\mathbf{D_{\ell}}$ are removed from our method. The number of output points for the \textit{global ghape} and \textit{local shape} ablations are kept consistent with our full method. 

% \input{tables/agg_ablation}
% \input{tables/emd_shapenet}
% \input{tables/kitti_metric}

We report the ablation results in Table~\ref{table:agg_ablation_sem_kitti}b on ShapeNet, as an average over all categories, and on Semantic KITTI. We find that all components of our system are crucial for optimal performance across both datasets. We further report the F-score@1\%~\cite{xie2020grnet} and the EMD metric on the Semantic KITTI dataset with the ablation of removing inpainting in Table \ref{table:kitti_agg_emd}c. We find that inpainting greatly improves our results across both of these metrics.

%We find that multi-view training and inpainting significantly impact the performance on the ShapeNet dataset. Whereas, the multi-scale encoding greatly improves the accuracy on KITTI.



% The qualitative effects of each part of our pipeline can be seen in Figure~\ref{fig:ablation_results}. We find that inpainting helps to align the predicted points to the input shape rather than aligning to the average shape across the dataset.

%%%%%%%%% NEW
The qualitative effects of our ablation study can be seen in Figure~\ref{fig:ablation_results}. We observe that inpainting generates an object-specific, less noisy output, when comparing "Ours" and "Without Inpainting". Our method without local loss fails to complete local details of an object such as back of a car or wings of a plane and without the global loss predicts a generic, noisy shape of an object. Since each local encoder and decoder only observe the points within that region and not the points in the other potentially occluded regions, they allow the network to focus on individual parts of an object and be robust to different occlusion patterns. The local loss helps in creating a more uniform completion, since it completes its associated region and the global loss reasons about the entire shape of the object. Finally, without multi-view loss, the output point cloud is noisy and incomplete as can be seen in all shapes.
%%%%%%%%%

%%%%%%%%% OLD
% The qualitative effects of each part of our pipeline can be seen in Figure~\ref{fig:ablation_results}. We observe that inpainting generates an object-specific point cloud and produces less noise on comparing ``Ours~(Full)" and ``Without Inpainting." Our method without local loss fails to complete the local details of an object such as the back of the car or the wings of the plane and without the global loss predicts a generic, noisy shape of each object. Local encoders and decoders allow the network to focus on individual parts of an object and be robust to different occlusion patterns, since each encoded region only observes the points within that region and not the points in the other potentially occluded regions. The local loss forces the network to create a more uniform completion, since it is responsible for completing its associated region. The global loss allows our method to reason about the entire shape of the object.
%%%%%%%%%

%also prevent the network from focusing on only densifying unoccluded regions, as the loss cannot be reduced by moving their associated points out of their region into unoccluded regions, where ground truth points are more likely. 

%We believe that the local encoding increases the density of points generated in the occluded regions since the local decoder and local shape loss ensure that points are generated in each region of the output space.

% \input{images/pose_noise_results}


%\begin{figure}[t]
% 	\centering
% 	\includegraphics[width=\columnwidth]{figures/pose_noise_results_bar.pdf}
% 	\caption{Mean of the Chamfer distance across all ShapeNet categories (Airplane, Car, Chair). Our method is trained with noisy poses, with and without inpainting, shown in \textcolor{green}{green} and \textcolor{red}{red}, respectively. The Gu~\etal~\cite{gu2020weakly} baseline is trained and tested with zero noise.} 
% 	\label{fig:pose_noise_results_bar}
%\end{figure}
% \input{tables/cd_emd_fig_table}
% \vspace{-1em}
% \subsection{Discussion}
\vspace{-1.125em}
\subsection{Robustness to Canonical Frame Estimation}
\vspace{-0.5em}
\label{sec:robustness}
%%%%%%%%%% NEW
Previous work~\cite{gu2020weakly} depends on multiple views which can be sensitive to the pose alignment errors. While we also use a multi-view loss, our inpainting losses make the model robust to noisy alignment allowing it to learn from poorly aligned data. The mean rotation/translation difference, after using IT-Net for pose canonicalization, between the multiple partially observed shapes during both training and inference is $5.46^{\circ}/~0.008$, $12.33^{\circ}/~0.013$ and $7.12^{\circ}/~0.010$ for Car, Chair, and Plane, respectively~(unit of translation is object diameter). This shows that even the canonicalized poses are not perfectly aligned and due to inpainting, our method is still able to learn from this poorly aligned data (particularly with respect to rotation). To further highlight the contribution of inpainting to this robustness, we add noise to the predicted IT-Net poses with rotations and translations sampled uniformly with a maximum displacement of 5\textdegree / 0.01, 10\textdegree / 0.05, and 15\textdegree / 0.10. Figure in Table~\ref{table:kitti_agg_emd}a shows that without inpainting (in \textcolor{red}{red}), our method is extremely sensitive to alignment noise but with inpainting (in \textcolor{green}{green}), our method only degrades slightly with higher noise, and remains more accurate at all levels of noise than the baseline~\cite{gu2020weakly} with no noise added.
%%%%%%%%%%

\vspace{-1.125em}
\subsection{Impact of $\beta$ in the Weighted Chamfer Distance loss} 
\vspace{-0.5em}
% The two terms in the asymmetric Weighted Chamfer Distance loss, $\mathcal{L}_{wcd}$ contribute in different ways towards shape completion. The first term is helpful in spreading out the points to complete the shape in missing regions, whereas the second term brings the points closer to the input point cloud to ensure shape consistency with the input. We conduct an experiment  where we train PointPnCNet with different values of $\beta$ to further understand the impact of each term in completing the shape quantitatively. We report the results in Table~\ref{table:beta_table}a. 
\input{tables/beta_table_only}
% \input{tables/beta_table_only}
We present an analysis in Table~\ref{table:beta_table} in which we train PointPnCNet with different values of $\beta$ to understand the contribution of the second term in the asymmetric Weighted Chamfer Distance loss (Eqn.~\ref{equ:cd_global_loss}), $\mathcal{L}_{wcd}$.
%towards shape completion and report the results 
 
%The first term is helpful in spreading out the points to complete the shape in missing regions, whereas the second term brings the points closer to the input point cloud to ensure shape consistency with the input. 

% \input{tables/beta_remove_portion}

From Table~\ref{table:beta_table}, we can observe that 
the optimal performance occurs at $\beta = 0.25$ across both the ShapeNet and KITTI datasets.
Our intuition is that a larger value of $\beta$ imposes a penalty for generating points in $Y$ in the regions that were occluded in the input; this contradicts our goal of completing those missing regions.  Nonetheless, setting $\beta = 0$ also leads to worse performance because the second term in Eqn.~\ref{equ:cd_global_loss} is needed to (minimally) penalize the network for predicting points in $Y$ that are far from the original partial point cloud $X$. Setting $\beta = 0.25$ provides the appropriate balance between these competing objectives.  As explained in Section~\ref{sec:losses}, this tradeoff only occurs for the global loss; the local loss uses a regional indicator that only applies the loss to regions for which we have ground truth information.

% the performance significantly deteriorates when $\beta=0$. This is because while the first term spreads out the points in the space, due to the absence of second term at $\beta=0$, the network is not incentivized to keep the points within the input space. 

%The network performs optimally with $\beta=0.25$ but the performance reduces again with higher $\beta$ value. 

% A higher $\beta$ imposes a large penalty on the output points in the missing regions that brings the points unnecessarily closer to the input point cloud. 

%This in turn negatively impacts the ability of the model to complete the shape and hence, reduces the performance. $\beta$ keeps a balance between completing the shape, down-weighting the penalty caused by the second term, and ensuring shape consistency with the input point cloud. A small value of $\beta$ prevents the second term from forcing all the points onto the input point cloud while ensuring that the points are well distributed to fully complete the shape. This is particularly important for allowing Inpainting Global Loss to ensure shape consistency while preventing it from negatively pulling the output points closer to the input.



% From Table~\ref{table:beta_table}a, we can observe that the performance significantly deteriorates when $\beta=0$. This is because while the first term enables the points to be spread out in the space, due to the absence of second term at $\beta=0$, the network is not incentivized to keep the points within the input space. The network performs optimally with $\beta=0.25$ but the performance reduces again with higher $\beta$ value. A higher $\beta$ imposes a large penalty on the output points in the missing regions that brings the points unnecessarily closer to the input point cloud. This in turn negatively impacts the ability of the model to complete the shape and hence, reduces the performance. 




% To further understand the contribution and impact of each loss component in Equation~\ref{equ:cd_global_loss} on shape completion, we conduct an experiment where we train PointPnCNet with different values of $\beta$. We report the results in Table~\ref{table:beta_table}a. 
% We perform an analysis on the different values of beta and report the results in Table Table~\ref{table:beta_table}a. These results emphasize the contribution of each term in Equation~\ref{equ:cd_global_loss} in completing the shape. The first term is helpful in spreading out the points to complete the shape in missing regions, whereas the second term brings the points closer to the input point cloud to ensure shape consistency with the input.

% From the results in Table~\ref{table:beta_table}, it can be observed that increasing the value of beta degrades the network’s performance. This is because a large penalty is applied to the output points in the missing regions that brings the points closer to the input point cloud, which in turn, affects the completed shape and the network’s performance.

% Moreover, at beta = 0, the network’s performance is negatively affected because the first term spreads the points in the space and the network is not incentivized to keep the points within the input space. Beta keeps a balance between completing the shape,  down-weighting the penalty caused by the second term, and ensuring shape consistency with the input point cloud. A small value of beta prevents the second term from forcing all the points onto the input point cloud but also ensures that the points are well distributed such that they can  fully complete the shape.
%%%%%%% here - Sectio 4.8
% \vspace{-1.125em}
% \subsection{Performance Analysis with respect to Occlusions}
% \vspace{-0.5em}
% We conduct an experiment to assess the impact of occlusions in the input partial point clouds on the ability of the model to complete the given shape. To do so, we introduce artificial occlusions by removing a certain number of regions from the input during testing (we have divided the input into 8 total regions). Given that the original input is already naturally occluded, we artificially remove at most three regions because beyond that, the input is barely visible. The results are shown in  Table~\ref{table:beta_table}b; we can observe that as the number of artificial occlusions in the input increases, there is a slight drop in performance for all categories. However, the model is considerably robust to the additional occlusions.
%%%%%%% here - Sectio 4.8

%%%%%%%%%% OLD 
% Previous work~\cite{gu2020weakly} depends on multiple viewpoints which can be sensitive to the pose alignment; while we also use a multi-viewpoint loss, we use an inpainting loss that considers a single viewpoint and is thus robust to noisy alignment.  To validate this claim, we evaluate the consistency of the IT-Net~\cite{yuan2018iterative} alignments. The mean rotation/translation difference between the multiple partially observed shapes, after using IT-Net for pose canonicalization, is $5.46^{\circ}/0.008$, $12.33^{\circ}/0.013$ and $7.12^{\circ}/0.010$ for Car, Chair, and Plane, respectively (translation is the multiple of object diameter). This shows that estimated canonicalized poses used in both training and inference are not perfectly aligned, particularly with respect to rotation; nonetheless, our method is able to learn from this poorly aligned data and is thus robust to some amount of alignment noise. As a further analysis of sensitivity of our method to the alignment error, we add noise to the predicted poses of IT-Net  with rotations and translations sampled uniformly with a maximum displacement of 5\textdegree / 0.01, 10\textdegree / 0.05, and 15\textdegree / 0.10, respectively (translations measured as multiples of the object diameter). We compare our method, with and without inpainting, shown in green and red on figure in Table~\ref{table:kitti_agg_emd}a, respectively. We observe that without inpainting, our method is extremely sensitive to alignment noise. However, with inpainting, our method only degrades slightly from higher alignment noise, and remains more accurate at all levels of noise than the baseline with no noise added~\cite{gu2020weakly}. This emphasizes that our method can operate with some amount of noisy alignment as compared to the previous multi-view approach.
%%%%%%%%%%

%From the Figure~\ref{fig:pose_noise_results}, it can be observed that after addition of some amount of noise, our method is able to perform better than the baseline~\cite{gu2020weakly} (gray dashed line, no noise was added to the baseline) emphasizing the robustness of our method towards noisy pose predictions. We also perform this analysis on our method with and without inpainting. It can be seen that.....



%It additionally incentivizes the network to place points in regions not occupied by the input cloud.
%inpainting helps to distribute the points away from the input cloud, fully covering the target shape.
% The local encoding appears to increase the density of point generated in the occluded regions. This is likely due to
% the local decoder and local shape loss ensuring that points are generated in each region of the output space. %analyze the different ablation experiments qualitatively by visualization the point clouds generated by the different experiments across different categories of ShapeNet and Semantic KITTI dataset. Figure [] portrays these visualizations.


% \subsection{Number of views}

% We evaluate the sensitivity of our multi-view loss to the number of views available at training time in Table~\ref{tbl:views}. In our base method, we use 4 views. We minimise the number of views to 2 views and 3 views and report its results on the Shapenet and KITTI dataset. It can be observed that our model is able to outperform the baseline with 2 views and 3 views as well stating that PointPnCNet is able to work on even lower amount of available data. We also show the qualtitative results on 2 views and 3 views in the Figure~\ref{fig:views_results}.


%present our results on the number of views used during the network training in Table~\ref{tbl:views}. In our base method, we use 4 views. We minimise the number of views to 2 views and 3 views and report its results on the Shapenet and KITTI dataset. It can be observed that our model is able to outperform the baseline with 2 views and 3 views as well stating that PointPnCNet is able to work on even lower amount of available data.%
%partitioning the space, using multi-resolution encoders and decoder, and other individual novel aspects of our method PointPnCNet, we conduct an extensive ablation study based on three major novel components of our approach -- architecture type, presence/absence of inpainting and application of overlapping grid boundaries. \ref{tbl:ablation_shapenet} and \ref{table:kitti_ablation} summarizes the results and findings of the ablation experiments we conduct.



% To evaluate the importance of each component in our method, we present an exhaustive ablation study on the basis of three components - architecture style, presence/absence of inpainting, and fuzzy boundaries. \ref{tbl:ablation_shapenet} and \ref{table:kitti_ablation} show a comparison with different combinations of encoders and decoders on the Shapenet and Semantic KITTI dataset highlighting the importance of the architecture combination of PointPnCNet. 

% We also present a qualitative analysis of each component in Figure.

% quantitative 

% qualitative



%\subsection{Discussion}
%\brian{These are likely supplementary results}
%In this section, we discuss some of the salient aspects of our approach and provide further insights into the working of PointPnCNet.

%\paragraph{Trend in performance with different number of views} We also evaluate our method by limiting the number of views used in the training. In Table, we present the performance of our method on 2 views and 3 views.

%\paragraph{Comparison to view aggregation} With the ground truth annotations present in Shapenet, we combine the 4 partial views of an object and calculate the Chamfer distance metric with the corresponding ground truth and present the results in Table. Through this analysis, we are able to show that our network is able to learn to complete the point cloud and generate a shape which is even better than just combining the given multiple views of an object. 

%\paragraph{Per point chamfer distance analysis} We also analyse the pointwise Chamfer metric of our method by generating a heatmap on both the datasets. We compare the heatmap of our method with the baselines and our ablations. 

% \paragraph{Extension to more fine-grained lower resolution grids} Lastly, we also analyse the importance of hierarchy by adding one more level of partitioning in our model. We partition the input partial point cloud in a ${3\times 3\times 3}$ and present the results in Table. We observe that the network gives a performance which is similar to our current model. \dave{This should probably be moved to the appendix.  It doesn't really show the importance of hierarchy to add an extra layer and show that it doesn't make a difference.}

% We present a further analysis to evaluate the performance of our method. With the ground truth annotations present in Shapenet, we combine the 4 partial views of an object and calculate the chamfer distance metric with the corresponding ground truth and present the results in Table. Through this analysis, we are able to show that our network is able to learn to complete the point cloud and generate a shape which is even better than just combining the given multiple views of an object. \himangi{Show Figure too}. 

%We also analyse the pointwise Chamfer metric of our method by generating a heatmap on both the datasets. We compare the heatmap of our method with the baselines and our ablations. 

%We also evaluate our method by limiting the number of views used in the training. In Table, we present the performance of our method on 2 views and 3 views.

%Lastly, we also analyse the importance of hierarchy by adding one more level of partitioning in our model. We partition the input partial point cloud in a ${3\times 3\times 3}$ and present the results in Table. We observe that the network gives a performance which is similar to our current model. 

% ground truth

% heat maps

% multiple views

% hierarchy


%\input{tables/shapenet_ablation}
%\input{tables/kitti_ablation}
%\input{tables/shapenet_views}
%\input{tables/shapenet_component_ablation}




==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/latex/5-conclusion.tex <==
\vspace{-1.5em}
\section{Conclusion}
\vspace{-0.5em}

%%%%%%% NEW
We propose a self-supervised method for point cloud completion via inpainting and random region removal that can be trained using only LiDAR-based partial point clouds. Our method produces significantly more accurate point cloud completions and outperforms the previous unsupervised methods on ShapeNet and Semantic KITTI. Through exhaustive ablation, we show the importance of each component of our method and the robustness to alignment errors. While the current method uses intersecting half-spaces defined by coordinate planes, other methods for point cloud partitioning can be explored in future work. We hope that our method will improve real-world 3D object understanding.
%%%%%%% 
\vspace{-1em}
\section{Acknowledgements}
\vspace{-0.5em}

This material is based upon work supported by the National Science Foundation under Grant No. IIS-1849154, and the CMU Argo AI Center for Autonomous Vehicle Research.
%%%%%%% OLD
% In this work, we propose a self-supervised method for point cloud completion through random region removal and inpainting. Our method achieves state-of-the-art performance across multiple object categories of ShapeNet and Semantic KITTI. We demonstrate that our method can be trained using only the partial point clouds of LiDAR sensors in autonomous driving scenarios and produces significantly more accurate point cloud completions than previous methods. We show extensive ablations demonstrating the importance of each component of our method and also show that our method is robust to alignment errors. We hope that our method will enable better 3D understanding of objects in the real-world.
%%%%%%% 

% \vspace{-1.5em}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/agg_ablation.tex <==
%\begin{table}[t]
%\smaller
%\begin{tabular}{l|c|cccc}
% & & \multicolumn{4}{c}{Model without} \\
% Dataset & Baseline & Inpainting & Multi-view & Global & Local \\
%\hline
%ShapeNet & 2.28 & 3.26 & 3.29 & 2.78 & 2.60 \\
% KITTI & 0.095 & 0.145 & 0.125 & 0.392 & 0.336 \\ 
%\end{tabular}
%\caption{Ablation Results on ShapeNet and KITTI Datasets with respect to Chamfer distance. ShapeNet %results are averaged across each object}
%\label{table:kitti_ablation}
%\end{table}

\begin{table}[h]
\small
\centering
\begin{tabular}{l|cccc} 
 & \multicolumn{4}{c}{\textbf{Model without}} \\ \cline{2-5}
  &  \textbf{Inpainting} & \textbf{Multi-View} & \textbf{Global} & \textbf{Local} \\
 \textbf{Dataset} & \textbf{Loss} & \textbf{Loss} & \textbf{Loss} & \textbf{Loss} \\
\hline\hline
%ShapeNet & -42.8\% & -44.2\% & -22.1\% & -14.0\% \\
%KITTI & -52.6\% & -30.6\% & -312.6\% & -254.7\% \\ 
ShapeNet & +0.98 & +0.27 & +0.50 & +0.32 \\
KITTI & +0.05 & +0.03 & +0.30 & +0.24 \\ \hline
\end{tabular}
\caption{Increase in mean Chamfer distance on ShapeNet and KITTI datasets for various ablations of our method. ShapeNet results are averaged across each object}
\label{table:agg_ablation}
% \vspace{-1em}
% \vspace{-1em}
\end{table}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/beta_remove_portion.tex <==
\begin{wraptable}[17]{r}{6cm}
% \begin{table}[t]
\vspace{-14pt}
\tiny
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ c}
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{c|llll}
\textbf{$\beta$} & \multicolumn{1}{c}{\textbf{Airplane}} & \multicolumn{1}{c}{\textbf{Car}} & \multicolumn{1}{c}{\textbf{Chair}} & \multicolumn{1}{c}{\textbf{KITTI}} \\ \hline \hline
0    &      2.10                                 &      2.63                            &   3.02                                 &   0.132                              \\
0.25 &      \textbf{1.66}                                 &              \textbf{2.48 }                   &       \textbf{2.70}                             &          \textbf{0.095 }                         \\
0.5  &      2.31                                 &      3.00                            &       3.28                             &      0.121                              \\
0.75 &          2.59                             &              3.50                    &               3.78                     &              0.142                      \\
1    &      3.83                                 &  4.72                                &    4.95                                &         0.196                           \\ \hline
\end{tabular}} \\ \footnotesize{(a)} \\
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{c|llll}
\multirow{3}{*}{
\parbox{1.5cm}{\centering \textbf{Number of Regions Removed}}} & & & & \\  & \multicolumn{1}{c}{\textbf{Airplane}} & \multicolumn{1}{c}{\textbf{Car}} & \multicolumn{1}{c}{\textbf{Chair}} & \multicolumn{1}{c}{\textbf{KITTI}} \\
  & & & & \\ \hline \hline
0                      &    \textbf{1.66}                                   &        \textbf{2.48}                          &    \textbf{2.70}                                &      \textbf{0.095}                              \\
\hline
1                     &     1.67                                  &               2.50                   &          2.73                          &   0.097                                 \\
2                      &    1.76                                   &            2.60                      &         2.79                           &     0.100                               \\
3                      &    1.89                                   &             2.67                     &         2.95                           &       0.102                             \\
\hline
\end{tabular}} \\
 \footnotesize{(b)} \\
\end{tabular}
\caption{(a). Performance analysis on different values of hyperparameter $\beta$ used in Equation~\ref{equ:cd_global_loss}, (b). Chamfer Distance on Shapenet and KITTI with varying number of removed regions.}
\label{table:beta_table_old}
% \end{table}
\end{wraptable}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/beta_table_only.tex <==
% \begin{table}[]
% \begin{tabular}{c|cccc}
% Beta & \textbf{Airplane} & \textbf{Car}  & \multicolumn{1}{l}{\textbf{Chair}} & \multicolumn{1}{l}{\textbf{KITTI}} \\ \hline
% 0    & 2.10              & 2.63          & 3.02                               & 0.132                              \\
% 0.25 & \textbf{1.66}     & \textbf{2.48} & \textbf{2.70}                      & \textbf{0.095}                     \\
% 0.5  & 2.31              & 3.00          & 3.28                               & 0.121                              \\
% 0.75 & 2.59              & 3.50          & 3.78                               & 0.142                              \\
% 1    & 3.83              & 4.72          & 4.95                               & 0.196                              \\ \hline
% \end{tabular}
% \end{table}

\begin{wraptable}[9]{r}{6cm}
% \begin{table}[t]
\vspace{-14pt}
\tiny
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ c}
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{c|llll}
\textbf{$\beta$} & \multicolumn{1}{c}{\textbf{Airplane}} & \multicolumn{1}{c}{\textbf{Car}} & \multicolumn{1}{c}{\textbf{Chair}} & \multicolumn{1}{c}{\textbf{KITTI}} \\ \hline \hline
0    &      2.10                                 &      2.63                            &   3.02                                 &   0.132                              \\
0.25 &      \textbf{1.66}                                 &              \textbf{2.48 }                   &       \textbf{2.70}                             &          \textbf{0.095 }                         \\
0.5  &      2.31                                 &      3.00                            &       3.28                             &      0.121                              \\
0.75 &          2.59                             &              3.50                    &               3.78                     &              0.142                      \\
1    &      3.83                                 &  4.72                                &    4.95                                &         0.196                           \\ \hline
\end{tabular}} \\ 
% \footnotesize{(a)} \\
% \resizebox{0.45\textwidth}{!}{
% \begin{tabular}{c|llll}
% \multirow{3}{*}{
% \parbox{1.5cm}{\centering \textbf{Number of Regions Removed}}} & & & & \\  & \multicolumn{1}{c}{\textbf{Airplane}} & \multicolumn{1}{c}{\textbf{Car}} & \multicolumn{1}{c}{\textbf{Chair}} & \multicolumn{1}{c}{\textbf{KITTI}} \\
%   & & & & \\ \hline \hline
% 0                      &    \textbf{1.66}                                   &        \textbf{2.48}                          &    \textbf{2.70}                                &      \textbf{0.095}                              \\
% \hline
% 1                     &     1.67                                  &               2.50                   &          2.73                          &   0.097                                 \\
% 2                      &    1.76                                   &            2.60                      &         2.79                           &     0.100                               \\
% 3                      &    1.89                                   &             2.67                     &         2.95                           &       0.102                             \\
% \hline
% \end{tabular}} \\
%  \footnotesize{(b)} \\
\end{tabular}
\caption{Performance analysis on different values of hyperparameter $\beta$ used in Equation~\ref{equ:cd_global_loss}.}
\label{table:beta_table}
% \end{table}
\end{wraptable}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/cd_emd_fig_table.tex <==
% \begin{figure}[h]
%  	\centering
%  	\begin{floatrow}
%  	\includegraphics[width=0.5\columnwidth]{images/pose_noise_results_line_new2.pdf}
%  	\caption{Mean of the Chamfer distance across all ShapeNet categories (Airplane, Car, Chair). Our method is trained with noisy poses, with and without inpainting, shown in \textcolor{green}{green} and \textcolor{red}{red}, respectively. The baseline Gu~\etal~\cite{gu2020weakly} has no added noise.} 
% %  	\label{fig:pose_noise_results}
% %  	\vspace{-1em}
% \begin{table}[]
% \centering
% \begin{tabular}{c|ll}
% \textbf{Training Method} & \multicolumn{1}{c}{\textbf{F-score@1\%} $\uparrow$ } & \multicolumn{1}{c}{\textbf{EMD} $\downarrow$} \\ \hline \hline
%  \multicolumn{1}{l|}{PointPnCNet (Ours)}       &    \textbf{0.67}                                      &                         \textbf{0.45}      \\ 
%  \multicolumn{1}{l|}{Ours~w/o inpainting}           &            0.44                              &                 0.62                 \\
% \hline  
% \end{tabular}
% \caption{F-Score@1\% and Earth Mover Distance (EMD) results on the Semantic KITTI dataset. We evaluate these metrics on our method vs our ablation of without inpainting.}
% \label{table:kitti_metrics}
% % \vspace{-1em}
% \end{table}
%  	\end{floatrow}
% \end{figure}

\begin{table}[!h]
% \vspace{-1em}
\small
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ cc} 
\multirow{4}{*}[1em]{
% \begin{minipage}{0.5\textwidth}
      \includegraphics[width=0.4\textwidth]{images/pose_noise_results_line_new2_2.pdf}
% \end{minipage}
} &
\resizebox{0.4\textwidth}{!}{
\begin{tabular} {l|ccc}
\textbf{Training Method}    & \textbf{Airplane} & \textbf{Car} & \textbf{Chair} \\ \hline \hline
\multicolumn{1}{l|}{DPC \cite{insafutdinov2018unsupervised}} & 0.146 & 0.160 & 0.194 \\
\multicolumn{1}{l|}{PointPnCNet (Ours)} & \textbf{0.108}  &  \textbf{0.120} &  \textbf{0.140} \\ \hline
\end{tabular}
} \\
& \footnotesize{(b)} \\ \\
& \resizebox{0.4\textwidth}{!}{
\begin{tabular}{c|ll}
\textbf{Training Method} & \multicolumn{1}{c}{\textbf{F-score@1\%} $\uparrow$ } & \multicolumn{1}{c}{\textbf{EMD} $\downarrow$} \\ \hline \hline
 \multicolumn{1}{l|}{PointPnCNet (Ours)}       &    \textbf{0.67}                                      &                         \textbf{0.45}      \\ 
 \multicolumn{1}{l|}{Ours~w/o inpainting}           &            0.44                              &                 0.62                 \\
\hline  
\end{tabular}
}  \\ 
\footnotesize{(a)} & \footnotesize{(c)} \\
\end{tabular}
\caption{(a). Mean of the chamfer distance across ShapeNet categories (Airplane, Car, Chair). Our method is trained with noisy poses, with \& without inpainting, shown in \textcolor{green}{green} and \textcolor{red}{red}, respectively. Baseline Gu~\etal~\cite{gu2020weakly} has no added noise, (b). Earth Mover Distance (EMD) metric on Shapenet. Lower EMD is better, (c). F-Score@1\% and EMD metrics on Semantic KITTI. We evaluate them on our method vs our ablation of without inpainting.}
\vspace{-1.625em}
\label{table:kitti_agg_emd}
\end{table}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/emd_shapenet.tex <==
\begin{table}[h]
\centering
\begin{tabular} {l|ccc}
\textbf{Training Method}    & \textbf{Airplane} & \textbf{Car} & \textbf{Chair} \\ \hline \hline
\multicolumn{1}{l|}{DPC \cite{insafutdinov2018unsupervised}} & 0.146 & 0.160 & 0.194 \\
\multicolumn{1}{l|}{PointPnCNet (Ours)} & \textbf{0.108}  &  \textbf{0.120} &  \textbf{0.140} \\ \hline
\end{tabular}
\caption{Earth Mover Distance (EMD) results on Airplane, Cars, and Chairs categories of the Shapenet dataset. A lower EMD is better.}
\label{table:emd_shapenet}
% \vspace{-1em}
\end{table}



==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/kitti_main.tex <==
\begin{table}[h]
\small
\centering
\setlength{\tabcolsep}{1.5pt}
\begin{tabular} {l|ccc}
\textbf{Method} & \textbf{CD} & \textbf{Precision} & \textbf{Coverage} \\
\hline
\hline
\multicolumn{1}{l|}{Gu~\etal~\cite{gu2020weakly}} & 0.194 & 0.087 & 0.107 \\
\multicolumn{1}{l|}{Densified Input} & 0.130  & \textbf{0.025}  & 0.105   \\
\hline
\multicolumn{1}{l|}{PointPnCNet (Ours)} & \textbf{0.095}  &  0.045 &  \textbf{0.050} \\ \hline
\end{tabular}
\caption{Quantitative results on the Semantic KITTI dataset}
\vspace{-1em}
\label{table:kitti_main_results}
\end{table}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/kitti_metric.tex <==
\begin{table}[h]
\centering
\begin{tabular}{c|ll}
\textbf{Training Method} & \multicolumn{1}{c}{\textbf{F-score@1\%} $\uparrow$ } & \multicolumn{1}{c}{\textbf{EMD} $\downarrow$} \\ \hline \hline
 \multicolumn{1}{l|}{PointPnCNet (Ours)}       &    \textbf{0.67}                                      &                         \textbf{0.45}      \\ 
 \multicolumn{1}{l|}{Ours~w/o inpainting}           &            0.44                              &                 0.62                 \\
\hline  
\end{tabular}
\caption{F-Score@1\% and Earth Mover Distance (EMD) results on the Semantic KITTI dataset. We evaluate these metrics on our method vs our ablation of without inpainting.}
\label{table:kitti_metrics}
% \vspace{-1em}
\end{table}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/kitti_uniformity.tex <==
\begin{table}[]
\centering
\begin{tabular}{c||ll}
\hline
\textbf{p}      & \multicolumn{1}{c}{\textbf{w/o inpainting}} & \multicolumn{1}{c}{\textbf{Ours}} \\ \hline
\textbf{0.4\%} &    0.815                                &         0.750                          \\
\textbf{0.6\%} &    0.773                              &           0.658                          \\
\textbf{0.8\%} &    0.697                              &           0.527                         \\
\textbf{1.0\%} &    0.588                              &           0.496                         \\
\textbf{1.2\%} &    0.517                              &           0.384 \\
\hline
\end{tabular}
\caption{Uniformity Metric on the KITTI dataset compared with our baseline of our model without inpainting.}
\label{tbl:kitti_uniformity}
\end{table}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/more_ablations.tex <==

% \begin{table*}[t]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l||lll|lll|lll|lll}
% \multirow{2}{*}{\textbf{Ablation}} & \multicolumn{3}{c|}{\textbf{Airplane}}               & \multicolumn{3}{c|}{\textbf{Car}}                    & \multicolumn{3}{c|}{\textbf{Chair}}                  & \multicolumn{3}{c}{\textbf{KITTI}}                   \\ \cline{2-13} 
%                                   & \textbf{CD} & & \textbf{CD} & \textbf{CD} &  \textbf{CD} \\ \hline
% % \textbf{Different weights}                              & \multicolumn{1}{c}{1.680}       &      \multicolumn{1}{c}{0.780}              &            \multicolumn{1}{c|}{0.900}       &      \multicolumn{1}{c}{2.520}       &     \multicolumn{1}{c}{0.950}               &        \multicolumn{1}{c|}{1.560}           &    \multicolumn{1}{c}{2.810}         &      \multicolumn{1}{c}{1.410}              &  \multicolumn{1}{c|}{1.400}                 &   \multicolumn{1}{c}{0.117}          &  \multicolumn{1}{c}{0.061}                  &       \multicolumn{1}{c}{0.056}           \\
% \textbf{Features concatenation}                               & \multicolumn{1}{c}{1.670}        &    \multicolumn{1}{c}{2.500}     &           \multicolumn{1}{c}{2.820}      &    \multicolumn{1}{c}{0.105}       \\
% % \textbf{Removal of overlapping region}                               & \multicolumn{1}{c}{1.690}        &       \multicolumn{1}{c}{0.820}             &      \multicolumn{1}{c|}{0.870}             &    \multicolumn{1}{c}{2.500}         &  \multicolumn{1}{c}{1.000}                  & \multicolumn{1}{c|}{1.500}                  &     \multicolumn{1}{c}{2.740}        &    \multicolumn{1}{c}{1.400}               &   \multicolumn{1}{c|}{1.340}                &       \multicolumn{1}{c}{0.096}      &     \multicolumn{1}{c}{0.042}               &       \multicolumn{1}{c}{0.054}           \\
% \textbf{Adding more levels}                               & \multicolumn{1}{c}{3.03}        &     \multicolumn{1}{c}{2.55}    &       \multicolumn{1}{c}{2.07}      &       \multicolumn{1}{c}{0.123}    \\
% \textbf{Our Full Method}                               & \multicolumn{1}{c}{\textbf{1.660}}        &                      \multicolumn{1}{c}{\textbf{2.480}}        &     \multicolumn{1}{c}{\textbf{2.700}}        &    \multicolumn{1}{c}{\textbf{0.095}}                 \\
% \end{tabular}
% }
% \caption{Quantitative Results on the architectural changes in our method. All the values reported for Shapenet are multiplied with 100.}
% \label{tbl:more_ablations}
% \end{table*}

\begin{table}[]
\centering
{%
\begin{tabular}{c||cccc}
\hline
\multirow{2}{*}{\textbf{Ablation}} & \multicolumn{1}{c|}{\textbf{Airplane}} & \multicolumn{1}{c|}{\textbf{Car}} & \multicolumn{1}{c|}{\textbf{Chair}} & \textbf{KITTI}       \\ \cline{2-5} 
                                   & \multicolumn{1}{c|}{\textbf{CD}}       & \multicolumn{1}{c|}{\textbf{CD}}  & \multicolumn{1}{c|}{\textbf{CD}}    & \textbf{CD}          \\ \hline
\multicolumn{1}{l||}{\textbf{Adding third level}}                                  & \multicolumn{1}{c|}{2.070}        &     \multicolumn{1}{c|}{2.550}    &       \multicolumn{1}{c|}{3.030}      &       \multicolumn{1}{c}{0.123}    \\
\multicolumn{1}{l||}{\textbf{Our method~(2 levels)}}                                  & \multicolumn{1}{c|}{\textbf{1.660}}        &                      \multicolumn{1}{c|}{\textbf{2.480}}        &     \multicolumn{1}{c|}{\textbf{2.700}}        &    \multicolumn{1}{c}{\textbf{0.095}}                 \\
\hline
\end{tabular}
}
\caption{Quantitative Results on the architecture changes in our method. All the Chamfer Distance metric values reported for Shapenet are multiplied with 100. It can be observed that adding a third level does not give a significant improvement in the performance.}
\label{tbl:more_ablations}
\end{table}



==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/num_occlusions.tex <==
\begin{table}[]
\centering
\begin{tabular}{c|cccc}
\textbf{\begin{tabular}[c]{@{}c@{}}Number of regions\\ removed\end{tabular}} & \textbf{Airplane} & \textbf{Car}  & \textbf{Chair} & \textbf{KITTI} \\ \hline \hline
0                                                                            & \textbf{1.66}     & \textbf{2.48} & \textbf{2.70}  & \textbf{0.095} \\ \hline
1                                                                            & 1.67              & 2.50          & 2.73           & 0.097          \\
2                                                                            & 1.76              & 2.60          & 2.79           & 0.100          \\
3                                                                            & 1.89              & 2.67          & 2.95           & 0.102   \\      \hline
\end{tabular}
\caption{Chamfer Distance onShapenet and KITTI with varying numberof removed regions}
\label{tbl:num_region}
\end{table}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/obs_unobs.tex <==
\begin{table}[]
\centering
{
\begin{tabular}{c||cccc}
\hline
\multicolumn{1}{l||}{\textbf{Region}} & \multicolumn{1}{l}{\textbf{Airplane}} & \multicolumn{1}{l}{\textbf{Car}} & \multicolumn{1}{l}{\textbf{Chair}} & \multicolumn{1}{l}{\textbf{KITTI}} \\ \hline
\textbf{Observed Precision} &    \multicolumn{1}{c}{0.771}                                    &     \multicolumn{1}{c}{1.113}                               &             \multicolumn{1}{c}{1.767}                     &  \multicolumn{1}{c}{0.625}                                  \\
\textbf{Unobserved Precision}   &        \multicolumn{1}{c}{0.824}                                &    \multicolumn{1}{c}{1.127}                                 &     \multicolumn{1}{c}{1.844}                             &        \multicolumn{1}{c}{0.640}                            \\
\textbf{Observed Coverage}  &  \multicolumn{1}{c}{0.848}                                      &  \multicolumn{1}{c}{1.490}                                  &   \multicolumn{1}{c}{1.344}                               &     \multicolumn{1}{c}{0.531}                               \\
\textbf{Unobserved Coverage}    &       \multicolumn{1}{c}{0.857}                                 &      \multicolumn{1}{c}{1.496}                               &    \multicolumn{1}{c}{1.355}                              &   \multicolumn{1}{c}{0.648}   \\
\hline
\end{tabular}
}
\caption{Precision and Coverage for the observed and unobserved regions on the Shapenet and KITTI dataset.}
\label{tbl:obs_unobs}
\end{table}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/pcn_sup_self_sup.tex <==
% \begin{table}[]
% \begin{tabular}{l||lll}
% \hline
% \multicolumn{1}{c||}{\textbf{Category}} & \multicolumn{1}{c}{\textbf{PCN (Fully supervised)}} & \multicolumn{1}{c}{\textbf{Ours (w/o inpainting)}} & \multicolumn{1}{c}{\textbf{Ours (Self-Supervised)}} \\ \hline
% \textbf{Airplane}                             &   0.0387                                                  &                                                    &                                                     \\
% \textbf{Cabinet}                             & 0.0707                                                    &                                                    &                                                     \\   
% \textbf{Car}                             & 0.0549                                                    &                                                    &                                                     \\
% \textbf{Chair}                             &  0.0680                                                   &                                                    &                                                     \\
% \textbf{Lamp}                             &                                                     &                                                    &                                                     \\
% \textbf{Sofa}                             &                                                     &                                                    &                                                     \\
% \textbf{Table}                             &                                                     &                                                    &                                                     \\
% \textbf{Vessel}                             &                                                     &                                                    &                                                     \\
% \hline
% \end{tabular}
% \end{table}

\begin{table}[]
\setlength{\tabcolsep}{4pt}
\begin{tabular}{p{0.28\textwidth}||p{0.001\textwidth}p{0.001\textwidth}p{0.001\textwidth}p{0.001\textwidth}p{0.001\textwidth}p{0.001\textwidth}p{0.001\textwidth}p{0.001\textwidth}}
\hline
\multicolumn{1}{l||}{\textbf{}}  & \multicolumn{1}{c}{\footnotesize{\textbf{Airplane}}} & \multicolumn{1}{c}{\footnotesize{\textbf{Cabinet}}} & \multicolumn{1}{c}{\footnotesize{\textbf{Car}}} & \multicolumn{1}{c}{\footnotesize{\textbf{Chair}}} & \multicolumn{1}{c}{\footnotesize{\textbf{Lamp}}} & \multicolumn{1}{c}{\footnotesize{\textbf{Sofa}}} & \multicolumn{1}{c}{\footnotesize{\textbf{Table}}} & \multicolumn{1}{c}{\footnotesize{\textbf{Vessel}}} \\ \hline
\textbf{\small{Ours~(w/o inpainting)}}  &   0.026                   &    0.045                            &   \multicolumn{1}{c}{0.031}                              &    0.039                            &    0.041                            &  \multicolumn{1}{l}{0.039}                               &      \multicolumn{1}{l}{0.040}                            &     \multicolumn{1}{l}{0.033}                            \\
\textbf{\small{Ours~(Self-Supervised)}} &  0.016                 &     0.027                           &    \multicolumn{1}{l}{0.024}                         &   0.027                             &  0.030                               &     \multicolumn{1}{l}{0.029}                          &    \multicolumn{1}{l}{0.025}                    &  \multicolumn{1}{l}{0.026}  \\
\hline
\textbf{\small{PCN (Fully Supervised)\cite{yuan2018pcn}}} &    0.005                 &  0.010                             &    \multicolumn{1}{c}{0.008}                            &    {0.010}                           &       {0.011}                         &   \multicolumn{1}{l}{0.011}                             &  \multicolumn{1}{l}{0.008}                              &     \multicolumn{1}{l}{0.009}                          \\
\hline
\end{tabular}
\caption{Quantitative results of comparison of our self-supervised method~(Ours) with fully supervised method, PCN~\cite{yuan2018pcn}, and ablation of our method without inpainting.}
\label{tbl:pcn_sup_self_sup}
\end{table}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/shapenet_ablation.tex <==
% \begin{table*}[h]
% \centering
% \footnotesize
% \setlength\tabcolsep{2pt}
% \begin{tabular}{c|c|c|c||c|c|c}
% \textbf{$E_{1^3}$} & \textbf{$E_{2^3}$} & \textbf{$D_{1^3}$} & \textbf{$D_{2^3}$} & \textbf{Airplane} &\textbf{ Car} & \textbf{Chair} \\ 
% \hline \hline
% \checkmark & & \checkmark & & &  &  \\ 
% \checkmark & & & \checkmark  &  &  &  \\
% \checkmark & & \checkmark & \checkmark  &  &  &  \\
% \hline
%  & \checkmark & \checkmark &  &  &  &  \\
%  & \checkmark &  & \checkmark &  &  &  \\
%  & \checkmark & \checkmark & \checkmark  &  &  &  \\
%  \hline
% \checkmark & \checkmark & \checkmark &  &  &  &  \\
% \checkmark & \checkmark &  & \checkmark &  &  &  \\
% \end{tabular}
% \caption{Ablation analysis: We study the effect of the different architecture styles on the the different cateogories of Shapenet dataset. Note: $1^3: 1 \times 1 \times 1$ and $2^3: 2 \times 2 \times 2$}\label{tbl:ablation_shapenet}
% \vspace{-1em}
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]

% \begin{tabular}{llll||lll|lll|lll}
% \hline
% \multicolumn{1}{c}{\multirow{2}{*}{$E_{1}$}} & \multicolumn{1}{c}{\multirow{2}{*}{$E_{2}$}} & \multicolumn{1}{c}{\multirow{2}{*}{$D_{1}$}} & \multicolumn{1}{c||}{\multirow{2}{*}{$D_{2}$}} & \multicolumn{3}{c|}{\textbf{Airplane}}        & \multicolumn{3}{c|}{\textbf{Car}}                                                                & \multicolumn{3}{c}{\textbf{Chair}}                                                    \\ \cline{5-13} 
% \multicolumn{1}{c}{}                     & \multicolumn{1}{c}{}                     & \multicolumn{1}{c}{}                     & \multicolumn{1}{c||}{}                     & \multicolumn{1}{c}{CD} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c|}{Coverage} & \multicolumn{1}{c}{CD} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c|}{Coverage} & \multicolumn{1}{c}{CD} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Coverage} \\ \hline
% \checkmark &  &  \checkmark  &              & \multicolumn{1}{c}{1.83} & \multicolumn{1}{c}{0.91} & \multicolumn{1}{c|}{0.92}  & \multicolumn{1}{c}{2.71} &   \multicolumn{1}{c}{1.12} & \multicolumn{1}{c|}{1.59}  &  \multicolumn{1}{c}{3.26} &\multicolumn{1}{c}{1.74} & \multicolumn{1}{c}{1.52}   \\ 
% \checkmark &  &              & \checkmark   & \multicolumn{1}{c}{1.93} & \multicolumn{1}{c}{0.92}  & \multicolumn{1}{c|}{1.01}  & \multicolumn{1}{c}{2.56} & \multicolumn{1}{c}{1.11}  &  \multicolumn{1}{c|}{1.45} &  \multicolumn{1}{c}{3.48}  &  \multicolumn{1}{c}{2.04} & \multicolumn{1}{c}{1.44}    \\ 
% \checkmark &  &  \checkmark  & \checkmark   & \multicolumn{1}{c}{1.82} & \multicolumn{1}{c}{0.92} & \multicolumn{1}{c|}{0.89} & \multicolumn{1}{c}{2.58} & \multicolumn{1}{c}{1.13}  & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c}{3.32} & \multicolumn{1}{c}{1.96}  & \multicolumn{1}{c}{1.45}   \\ 
% \hline
%           & \checkmark  &  \checkmark  &              &    \multicolumn{1}{c}{1.95}   &  \multicolumn{1}{c}{0.99} &   \multicolumn{1}{c|}{0.96} &   \multicolumn{1}{c}{2.79} &  \multicolumn{1}{c}{1.21}  &  \multicolumn{1}{c|}{1.58}  &   \multicolumn{1}{c}{3.52} &  \multicolumn{1}{c}{1.99} &  \multicolumn{1}{c}{1.53}   \\ 
%           & \checkmark  &              & \checkmark   &   \multicolumn{1}{c}{2.01}    &  \multicolumn{1}{c}{1.00} &  \multicolumn{1}{c|}{1.01} &    \multicolumn{1}{c}{2.61}   &  \multicolumn{1}{c}{1.19}  &  \multicolumn{1}{c|}{\textbf{1.42}}  &    \multicolumn{1}{c}{3.73}    &  \multicolumn{1}{c}{2.30} &  \multicolumn{1}{c}{1.43}   \\ 
%           & \checkmark  &  \checkmark  & \checkmark   &  \multicolumn{1}{c}{1.93}    & \multicolumn{1}{c}{1.00} & \multicolumn{1}{c|}{0.93} &  \multicolumn{1}{c}{2.65}    &  \multicolumn{1}{c}{1.20} & \multicolumn{1}{c|}{1.45}  &  \multicolumn{1}{c}{3.61}     & \multicolumn{1}{c}{2.22}  & \multicolumn{1}{c}{1.39}    \\ 
% \hline                         
% \checkmark & \checkmark &  \checkmark  &              & \multicolumn{1}{c}{1.86} &  \multicolumn{1}{c}{0.80} & \multicolumn{1}{c|}{1.06} & \multicolumn{1}{c}{2.84} & \multicolumn{1}{c}{\textbf{0.94}}  & \multicolumn{1}{c|}{1.90}  &  \multicolumn{1}{c}{3.11} & \multicolumn{1}{c}{\textbf{1.33}} & \multicolumn{1}{c}{1.78}   \\  
% \checkmark & \checkmark &              & \checkmark   & \multicolumn{1}{c}{1.85} & \multicolumn{1}{c}{0.82} & \multicolumn{1}{c|}{1.03} & \multicolumn{1}{c}{2.53} & \multicolumn{1}{c}{0.96}  & \multicolumn{1}{c|}{1.57}  &  \multicolumn{1}{c}{3.25} & \multicolumn{1}{c}{1.76}  & \multicolumn{1}{c}{1.49}   \\ 
% \checkmark & \checkmark & \checkmark   & \checkmark   & \multicolumn{1}{c}{\textbf{1.66}} & \multicolumn{1}{c}{\textbf{0.79}} & \multicolumn{1}{c|}{\textbf{0.87}} & \multicolumn{1}{c}{\textbf{2.48}} & \multicolumn{1}{c}{0.99}  & \multicolumn{1}{c|}{1.49}  &  \textbf{2.70} &  \multicolumn{1}{c}{1.36} &  \multicolumn{1}{c}{\textbf{1.34}} \\  
% \hline
% \end{tabular}

% \end{table*}

% \begin{table*}[]
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llll|lll|lll|lll|lll}
% \hline
% \multirow{2}{*}{\multirow{2}{*}{$E_{1}$}} & \multirow{2}{*}{\multirow{2}{*}{$E_{2}$}} & \multirow{2}{*}{\multirow{2}{*}{$D_{1}$}} & \multirow{2}{*}{\multirow{2}{*}{$D_{2}$}} & \multicolumn{3}{c|}{\textbf{Airplane}}               & \multicolumn{3}{c|}{\textbf{Car}}                    & \multicolumn{3}{c|}{\textbf{Chair}}                  & \multicolumn{3}{c}{\textbf{KITTI}}                   \\ \cline{5-16} 
%                               &                               &                               &                               & \textbf{CD} & \textbf{Precision} & \textbf{Coverage} & \textbf{CD} & \textbf{Precision} & \textbf{Coverage} & \textbf{CD} & \textbf{Precision} & \textbf{Coverage} & \textbf{CD} & \textbf{Precision} & \textbf{Coverage} \\ \hline
% \checkmark &  &  \checkmark  &              & \multicolumn{1}{c}{1.83} & \multicolumn{1}{c}{0.91} & \multicolumn{1}{c|}{0.92}  & \multicolumn{1}{c}{2.71} &   \multicolumn{1}{c}{1.12} & \multicolumn{1}{c|}{1.59}  &  \multicolumn{1}{c}{3.26} &\multicolumn{1}{c}{1.74} & \multicolumn{1}{c|}{1.52}  & \multicolumn{1}{c}{0.336}  &  \multicolumn{1}{c}{0.172}  & \multicolumn{1}{c}{0.164}    \\ 
% \checkmark &  &              & \checkmark   & \multicolumn{1}{c}{1.93} & \multicolumn{1}{c}{0.92}  & \multicolumn{1}{c|}{1.01}  & \multicolumn{1}{c}{2.56} & \multicolumn{1}{c}{1.11}  &  \multicolumn{1}{c|}{1.45} &  \multicolumn{1}{c}{3.48}  &  \multicolumn{1}{c}{2.04} & \multicolumn{1}{c|}{1.44}  & \multicolumn{1}{c}{1.042} & \multicolumn{1}{c}{0.305}   & \multicolumn{1}{c}{0.737}  \\ 
% \checkmark &  &  \checkmark  & \checkmark   & \multicolumn{1}{c}{1.82} & \multicolumn{1}{c}{0.92} & \multicolumn{1}{c|}{0.89} & \multicolumn{1}{c}{2.58} & \multicolumn{1}{c}{1.13}  & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c}{3.32} & \multicolumn{1}{c}{1.96}  & \multicolumn{1}{c|}{1.45}  & \multicolumn{1}{c}{0.357} &  \multicolumn{1}{c}{0.201}  & \multicolumn{1}{c}{0.156} \\ 
% \hline
%           & \checkmark  &  \checkmark  &              &    \multicolumn{1}{c}{1.95}   &  \multicolumn{1}{c}{0.99} &   \multicolumn{1}{c|}{0.96} &   \multicolumn{1}{c}{2.79} &  \multicolumn{1}{c}{1.21}  &  \multicolumn{1}{c|}{1.58}  &   \multicolumn{1}{c}{3.52} &  \multicolumn{1}{c}{1.99} &  \multicolumn{1}{c|}{1.53} & \multicolumn{1}{c}{0.329}   & \multicolumn{1}{c}{0.171}   & \multicolumn{1}{c}{0.158}  \\ 
%           & \checkmark  &              & \checkmark   &   \multicolumn{1}{c}{2.01}    &  \multicolumn{1}{c}{1.00} &  \multicolumn{1}{c|}{1.01} &    \multicolumn{1}{c}{2.61}   &  \multicolumn{1}{c}{1.19}  &  \multicolumn{1}{c|}{\textbf{1.42}}  &    \multicolumn{1}{c}{3.73}    &  \multicolumn{1}{c}{2.30} &  \multicolumn{1}{c|}{1.43} & \multicolumn{1}{c}{0.392}  &  \multicolumn{1}{c}{0.157}   &    \multicolumn{1}{c}{0.235}   \\ 
%           & \checkmark  &  \checkmark  & \checkmark   &  \multicolumn{1}{c}{1.93}    & \multicolumn{1}{c}{1.00} & \multicolumn{1}{c|}{0.93} &  \multicolumn{1}{c}{2.65}    &  \multicolumn{1}{c}{1.20} & \multicolumn{1}{c|}{1.45}  &  \multicolumn{1}{c}{3.61}     & \multicolumn{1}{c}{2.22}  & \multicolumn{1}{c|}{1.39}  & \multicolumn{1}{c}{0.362}   & \multicolumn{1}{c}{0.207} &    \multicolumn{1}{c}{0.155}  \\ 
% \hline                         
% \checkmark & \checkmark &  \checkmark  &              & \multicolumn{1}{c}{1.86} &  \multicolumn{1}{c}{0.80} & \multicolumn{1}{c|}{1.06} & \multicolumn{1}{c}{2.84} & \multicolumn{1}{c}{\textbf{0.94}}  & \multicolumn{1}{c|}{1.90}  &  \multicolumn{1}{c}{3.11} & \multicolumn{1}{c}{\textbf{1.33}} & \multicolumn{1}{c|}{1.78} & \multicolumn{1}{c}{0.388}   &    \multicolumn{1}{c}{0.175}  &    \multicolumn{1}{c}{0.213}   \\  
% \checkmark & \checkmark &              & \checkmark   & \multicolumn{1}{c}{1.85} & \multicolumn{1}{c}{0.82} & \multicolumn{1}{c|}{1.03} & \multicolumn{1}{c}{2.53} & \multicolumn{1}{c}{0.96}  & \multicolumn{1}{c|}{1.57}  &  \multicolumn{1}{c}{3.25} & \multicolumn{1}{c}{1.76}  & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c}{1.131}  &    \multicolumn{1}{c}{0.308}  & \multicolumn{1}{c}{0.823}   \\ 
% \checkmark & \checkmark & \checkmark   & \checkmark   & \multicolumn{1}{c}{\textbf{1.66}} & \multicolumn{1}{c}{\textbf{0.79}} & \multicolumn{1}{c|}{\textbf{0.87}} & \multicolumn{1}{c}{\textbf{2.48}} & \multicolumn{1}{c}{0.99}  & \multicolumn{1}{c|}{1.49}  &  \textbf{2.70} &  \multicolumn{1}{c}{1.36} &  \multicolumn{1}{c|}{\textbf{1.34}} & \multicolumn{1}{c}{\textbf{0.095}}   &    \multicolumn{1}{c}{\textbf{0.045}} & \multicolumn{1}{c}{\textbf{0.050}} \\  

% \hline
% \end{tabular}
% }
% \caption{Ablation analysis: We study the effect of the architecture styles through combinations of different number of encoders and decoders on the Airplane, Car, Chair of the Shapenet dataset and KITTI dataset.}
% \label{tbl:shapenet_ablation}
% \end{table*}


\begin{table}[hbt!]
\centering
{
\begin{tabular}{cccc||c|c|c|c}
\hline
\multirow{2}{*}{$E_{g}$} & \multirow{2}{*}{$E_{\ell}$} & \multirow{2}{*}{$D_{g}$} & \multirow{2}{*}{$D_{\ell}$} & \textbf{Airplane}         & \textbf{Car}          & \textbf{Chair}        & \textbf{KITTI}       \\ \cline{5-8} 
                              &                               &                               &                               & \textbf{CD}               & \textbf{CD}           & \textbf{CD}           & \textbf{CD}          \\ \hline
\checkmark &  &  \checkmark  &              & \multicolumn{1}{c|}{1.830} & \multicolumn{1}{c|}{2.710} &   \multicolumn{1}{c|}{3.260} & \multicolumn{1}{c}{0.336}  \\ 
\checkmark &  &              & \checkmark   & \multicolumn{1}{c|}{1.930} & \multicolumn{1}{c|}{2.560} &  \multicolumn{1}{c|}{3.480}  & \multicolumn{1}{c}{1.042} \\ 
\checkmark &  &  \checkmark  & \checkmark   & \multicolumn{1}{c|}{1.820} & \multicolumn{1}{c|}{2.580} & \multicolumn{1}{c|}{3.320} & \multicolumn{1}{c}{0.357} \\ 
\hline
& \checkmark  &  \checkmark  &              &    \multicolumn{1}{c|}{1.950}   &   \multicolumn{1}{c|}{2.790} &   \multicolumn{1}{c|}{3.520} & \multicolumn{1}{c}{0.329}   \\
& \checkmark  &              & \checkmark   &   \multicolumn{1}{c|}{2.010}    &    \multicolumn{1}{c|}{2.610}   &    \multicolumn{1}{c|}{3.730}    & \multicolumn{1}{c}{0.392}  \\
 & \checkmark  &  \checkmark  & \checkmark   &  \multicolumn{1}{c|}{1.930}    &  \multicolumn{1}{c|}{2.650}    &  \multicolumn{1}{c|}{3.610}     & \multicolumn{1}{c}{0.362}   \\
\hline
\checkmark & \checkmark &  \checkmark  &              & \multicolumn{1}{c|}{1.860} & \multicolumn{1}{c|}{2.840} &  \multicolumn{1}{c|}{3.110} & \multicolumn{1}{c}{0.388}   \\
\checkmark & \checkmark &              & \checkmark   & \multicolumn{1}{c|}{1.850} & \multicolumn{1}{c|}{2.530} &  \multicolumn{1}{c|}{3.250} & \multicolumn{1}{c}{1.131}  \\
\checkmark & \checkmark & \checkmark   & \checkmark   & \multicolumn{1}{c|}{\textbf{1.660}} & \multicolumn{1}{c|}{\textbf{2.480}} &  \multicolumn{1}{c|}{\textbf{2.700}} & \multicolumn{1}{c}{\textbf{0.095}}   \\  
\hline
\end{tabular}
}
\caption{We study the performance of the architecture styles through combinations of local and global encoders and decoders on the Airplane, Car, Chair of the Shapenet dataset and KITTI dataset via Chamfer Distance metric. It can be observed that a combination of global and local encoders and decoders gives the best performance among all the possible combinations.}
\label{tbl:shapenet_ablation}
\end{table}



==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/shapenet_f1score.tex <==
\begin{table}[]
\centering
\begin{tabular}{c||c|c|c}
\hline
 \textbf{Method} & \textbf{Airplane} & \textbf{Car} & \textbf{Chair} \\ \hline
\textbf{DPC\cite{insafutdinov2018unsupervised}}  &       0.423        &     0.364           &  0.315            \\
\textbf{Ours} &   \textbf{0.626}                &    \textbf{0.450}            &        \textbf{0.409}  \\   
\hline
\end{tabular}
\caption{F1-Score@1\% on the Shapenet dataset.}
\label{tbl:shapenet_f1score}
\end{table}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/shapenet_main.tex <==
% \begin{table*}[h]
% \centering
% \begin{tabular} {l|c c c}
% \textbf{Training Method} & \textbf{Airplane} & \textbf{Car} & \textbf{Chair} \\
% \hline
% \hline
% Weakly-Supervised & 1.95~/~0.91~/~1.05 & 2.68~/~1.27~/~1.41 & 3.33~/~1.69~/~1.64 \\
% Ours &  &  &  \\
% \end{tabular}
% \caption{Quantitative results on the Shapenet Dataset (Chamfer Metric~/~Precision~/~Coverage). All the reported values are multiplied by 100.}
% \vspace{-1em}
% \label{table:shapenet_main_results}
% \end{table*}

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc}
\multirow{2}{*}{\textbf{Method}}            & \multicolumn{3}{c|}{\textbf{Airplane}}                                                                              & \multicolumn{3}{c|}{\textbf{Car}}                                                                                   & \multicolumn{3}{c}{\textbf{Chair}}                                                                              \\ \cline{2-10} 
                                                     & \textbf{CD}                       & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c|}{\textbf{Coverage}} & \textbf{CD}                       & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c|}{\textbf{Coverage}} & \textbf{CD}                       & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Coverage}} \\ \hline \hline
 \multicolumn{1}{l|}{DPC \cite{insafutdinov2018unsupervised}}     & \multicolumn{1}{c}{3.91}                              & \multicolumn{1}{c}{-}               & \multicolumn{1}{c|}{-}              & \multicolumn{1}{c}{3.47}                              & \multicolumn{1}{c}{-}               & \multicolumn{1}{c|}{-}              & \multicolumn{1}{c}{4.30}                             & \multicolumn{1}{c}{-}              & \multicolumn{1}{c}{-}           \\                                         
\multicolumn{1}{l|}{Gu~\etal~\cite{gu2020weakly}}     & \multicolumn{1}{c}{1.95}                              & \multicolumn{1}{c}{0.91}               & \multicolumn{1}{c|}{1.05}              & 2.68                              & \multicolumn{1}{c}{1.27}               & \multicolumn{1}{c|}{\textbf{1.41}}              & 3.33                              & \multicolumn{1}{c}{1.69}               & \multicolumn{1}{c}{1.64}           \\ \hline
 \multicolumn{1}{l|}{PointPnCNet~(Ours)}                                & \multicolumn{1}{c}{\textbf{1.66}}          &    \multicolumn{1}{c}{\textbf{0.79}}                                  &         \multicolumn{1}{c|}{\textbf{0.87}}                              & \multicolumn{1}{l}{\textbf{2.48}}          &                 \multicolumn{1}{c}{\textbf{0.99}}                       &    \multicolumn{1}{c|}{1.49}                                    & \multicolumn{1}{c}{\textbf{2.70}} &           \multicolumn{1}{c}{\textbf{1.36}}                             &            \multicolumn{1}{c}{\textbf{1.34}}                        \\ \hline
\end{tabular}
}
\caption{Quantitative results on the Airplane, Cars, and Chairs categories of the ShapeNet dataset. All results are multiplied by a factor of 100, following Gu~\etal~\cite{gu2020weakly}.}
\label{table:shapenet_main_results}
\vspace{-1em}
\end{table*}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/shapenet_pose_noise.tex <==
% \begin{table}[]
% \begin{tabular}{p{0.01\textwidth}p{0.08\textwidth}p{0.09\textwidth}|p{0.03\textwidth}p{0.03\textwidth}p{0.03\textwidth}}
% \textbf{Training Method} & \textbf{Rotation Noise (R)} & \textbf{Translation Noise (T)} & \multicolumn{1}{c}{\textbf{Airplane}} & \multicolumn{1}{c}{\textbf{Car}} & \multicolumn{1}{c}{\textbf{Chair}} \\ \hline \hline
% \multicolumn{1}{l}{Gu~\etal~\cite{gu2020weakly}} & 0 & 0 & \multicolumn{1}{c}{1.95} & \multicolumn{1}{c}{2.68} & \multicolumn{1}{c}{3.33} \\
% \hline
%  & $5^{\circ}$         & 0.01                 &    \multicolumn{1}{c}{1.89}                                   &    \multicolumn{1}{c}{2.51}                              &          \multicolumn{1}{c}{2.88}                          \\
% Ours & $10^{\circ}$         & 0.05                &          \multicolumn{1}{c}{1.90}                             &      \multicolumn{1}{c}{2.51}                            &  \multicolumn{1}{c}{2.93}                                  \\
%  & $15^{\circ}$        & 0.10                &        \multicolumn{1}{c}{1.94}                               &       \multicolumn{1}{c}{2.54}                           &    \multicolumn{1}{c}{2.98}                               
% \end{tabular}
% \end{table}


\begin{table}[]
\centering
\begin{tabular}{p{0.07\textwidth}|p{0.06\textwidth}p{0.09\textwidth}|p{0.06\textwidth}p{0.03\textwidth}p{0.03\textwidth}}
                         & \multicolumn{2}{c|}{Noise}                       &                   &              &                \\
\textbf{Training Method} & \textbf{Rotation (R)} & \textbf{Translation (T)} & \textbf{Airplane} & \textbf{Car} & \textbf{Chair} \\ \hline \hline
Gu et al                 & 0                     & 0                        & 1.95              & 2.68         & 3.33           \\ \hline
\multirow{3}{*}{Ours}    & 5                     & 0.01                     & 1.89              & 2.51         & 2.88           \\
                         & 10                    & 0.05                     & 1.90              & 2.51         & 2.93           \\
                         & 15                    & 0.1                      & 1.94              & 2.54         & 2.98  \\ \hline        
\end{tabular}
\caption{Chamfer Distance on the ShapeNet dataset for Airplane, Cars, and Chairs categories. We add a sampled noise to the predicted canonical pose for every partial point cloud. Rotation Noise depicts the noise sampled from [-R, R] degrees and translation noise sampled from [-T, T]. Translation is the  percent of object diameter. All results are multiplied by a factor of 100, following from Gu~\etal~\cite{gu2020weakly}.}
\label{table:shapenet_pose_noise}
\end{table}


==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/shapenet_uniformity.tex <==



\begin{table}[]
\centering
{
\begin{tabular}{c||cc|cccc}
\hline
\multicolumn{1}{l||}{} & \multicolumn{2}{c|}{\textbf{Airplane}}                                & \multicolumn{2}{c|}{\textbf{Cars}}                                     & \multicolumn{2}{c}{\textbf{Chairs}}                                  \\ \hline
\textbf{p}            & \multicolumn{1}{c}{\textbf{DPC \cite{insafutdinov2018unsupervised}}} & \multicolumn{1}{c|}{\textbf{Ours}} & \multicolumn{1}{c}{\textbf{DPC}} & \multicolumn{1}{c|}{\textbf{Ours}} & \multicolumn{1}{c}{\textbf{DPC}} & \multicolumn{1}{c}{\textbf{Ours}} \\ \hline
\textbf{0.4\%}       &    \multicolumn{1}{c}{0.775}                              &    \multicolumn{1}{c|}{0.775}                               &    \multicolumn{1}{c}{0.758}                              & \multicolumn{1}{c|}{0.757}              &       \multicolumn{1}{c}{0.785}                           &       \multicolumn{1}{c}{0.787}                            \\
\textbf{0.6\%}       &       \multicolumn{1}{c}{0.674}                           &    \multicolumn{1}{c|}{0.673}                                &   \multicolumn{1}{c}{0.646}                               & \multicolumn{1}{c|}{0.647}              &     \multicolumn{1}{c}{0.664}                             &   \multicolumn{1}{c}{0.664}                                \\
\textbf{0.8\%}       &     \multicolumn{1}{c}{0.490}                             &     \multicolumn{1}{c|}{0.490}                               &     \multicolumn{1}{c}{0.489}                             & \multicolumn{1}{c|}{0.489}              &  \multicolumn{1}{c}{0.498}                                &      \multicolumn{1}{c}{0.497}                             \\
\textbf{1.0\%}       &       \multicolumn{1}{c}{0.395}                           &   \multicolumn{1}{c|}{0.394}                                 &    \multicolumn{1}{c}{0.388}                              & \multicolumn{1}{c|}{0.389}              &      \multicolumn{1}{c}{0.385}                            &    \multicolumn{1}{c}{0.385}                               \\
\textbf{1.2\%}       &    \multicolumn{1}{c}{0.256}                              &  \multicolumn{1}{c|}{0.257}                                  &  \multicolumn{1}{c}{0.246}                                & \multicolumn{1}{c|}{0.245}              &     \multicolumn{1}{c}{0.265}                             &     \multicolumn{1}{c}{0.264}                              \\ \hline
\end{tabular}
}
\caption{Uniformity Metric on the Shapenet dataset compared with the baseline DPC \cite{insafutdinov2018unsupervised}.}
\label{tbl:shapenet_uniformity}
\end{table}

==> BMVC21 ID_443-Self-Supervised Point Cloud Completion via Inpainting (Arxiv)/tables/table2_3.tex <==
% \begin{table}[h]
% \small
% \centering
% \begin{tabular}{l|cccc} 
%  & \multicolumn{4}{c}{\textbf{Model without}} \\ \cline{2-5}
%   &  \textbf{Inpainting} & \textbf{Multi-View} & \textbf{Global} & \textbf{Local} \\
%  \textbf{Dataset} & \textbf{Loss} & \textbf{Loss} & \textbf{Scale} & \textbf{Scale} \\
% \hline\hline
% %ShapeNet & -42.8\% & -44.2\% & -22.1\% & -14.0\% \\
% %KITTI & -52.6\% & -30.6\% & -312.6\% & -254.7\% \\ 
% ShapeNet & +0.98 & +0.61 & +0.50 & +0.32 \\
% KITTI & +0.05 & +0.03 & +0.30 & +0.24 \\ \hline
% \end{tabular}
% \caption{Increase in mean Chamfer distance on ShapeNet and KITTI datasets for various ablations of our method. ShapeNet results are averaged across each object}
% \label{table:agg_ablation}
% % \vspace{-1em}
% % \vspace{-1em}
% \end{table}

\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ cc } 
\resizebox{0.4\textwidth}{!}{
\begin{tabular} {l|ccc}
\textbf{Method} & \textbf{CD} & \textbf{Precision} & \textbf{Coverage} \\
\hline
\hline
Gu~\etal~\cite{gu2020weakly} & 0.194 & 0.087 & 0.107 \\
Densified Input & 0.130  & \textbf{0.025}  & 0.105   \\
\hline
PointPnCNet (Ours) & \textbf{0.095}  &  0.045 &  \textbf{0.050} \\ \hline
% \label{table:kitti_main_results}
\end{tabular}} &
\resizebox{0.57\textwidth}{!}{
\begin{tabular}{l|cccc} 
 & \multicolumn{4}{c}{\textbf{Model without}} \\ \cline{2-5}
 \textbf{Dataset} &  \textbf{Inpainting} & \textbf{Multi-View Loss} & \textbf{Global Loss} & \textbf{Local Loss} \\
%  \textbf{Dataset} & \textbf{Loss} & \textbf{Loss} & \textbf{Scale} & \textbf{Scale} \\
\hline\hline
%ShapeNet & -42.8\% & -44.2\% & -22.1\% & -14.0\% \\
%KITTI & -52.6\% & -30.6\% & -312.6\% & -254.7\% \\ 
ShapeNet & +0.98 & +0.27 & +0.50 & +0.32 \\
KITTI & +0.05 & +0.03 & +0.30 & +0.24 \\ \hline

\end{tabular}}  \\
\footnotesize{(a)} & \footnotesize{(b)} \\
\end{tabular}
\caption{(a). Quantitative results on the Semantic KITTI dataset, (b). Increase in mean Chamfer distance on ShapeNet and KITTI datasets for various ablations of our method. ShapeNet results are averaged across each object category.}
\vspace{-1em}
\label{table:agg_ablation_sem_kitti}
\end{table}

==> images/pose_noise_results.tex <==
\begin{figure}[t]
 	\centering
 	\includegraphics[width=0.5\columnwidth]{images/pose_noise_results_line_new2.pdf}
 	\caption{Mean of the Chamfer distance across all ShapeNet categories (Airplane, Car, Chair). Our method is trained with noisy poses, with and without inpainting, shown in \textcolor{green}{green} and \textcolor{red}{red}, respectively. The baseline Gu~\etal~\cite{gu2020weakly} has no added noise.} 
 	\label{fig:pose_noise_results}
 	\vspace{-1em}
\end{figure}

==> tables/agg_ablation.tex <==
%\begin{table}[t]
%\smaller
%\begin{tabular}{l|c|cccc}
% & & \multicolumn{4}{c}{Model without} \\
% Dataset & Baseline & Inpainting & Multi-view & Global & Local \\
%\hline
%ShapeNet & 2.28 & 3.26 & 3.29 & 2.78 & 2.60 \\
% KITTI & 0.095 & 0.145 & 0.125 & 0.392 & 0.336 \\ 
%\end{tabular}
%\caption{Ablation Results on ShapeNet and KITTI Datasets with respect to Chamfer distance. ShapeNet %results are averaged across each object}
%\label{table:kitti_ablation}
%\end{table}

\begin{table}[h]
\small
\centering
\begin{tabular}{l|cccc} 
 & \multicolumn{4}{c}{\textbf{Model without}} \\ \cline{2-5}
  &  \textbf{Inpainting} & \textbf{Multi-View} & \textbf{Global} & \textbf{Local} \\
 \textbf{Dataset} & \textbf{Loss} & \textbf{Loss} & \textbf{Loss} & \textbf{Loss} \\
\hline\hline
%ShapeNet & -42.8\% & -44.2\% & -22.1\% & -14.0\% \\
%KITTI & -52.6\% & -30.6\% & -312.6\% & -254.7\% \\ 
ShapeNet & +0.98 & +0.27 & +0.50 & +0.32 \\
KITTI & +0.05 & +0.03 & +0.30 & +0.24 \\ \hline
\end{tabular}
\caption{Increase in mean Chamfer distance on ShapeNet and KITTI datasets for various ablations of our method. ShapeNet results are averaged across each object}
\label{table:agg_ablation}
% \vspace{-1em}
% \vspace{-1em}
\end{table}

==> tables/beta_remove_portion.tex <==
\begin{wraptable}[17]{r}{6cm}
% \begin{table}[t]
\vspace{-14pt}
\tiny
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ c}
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{c|llll}
\textbf{$\beta$} & \multicolumn{1}{c}{\textbf{Airplane}} & \multicolumn{1}{c}{\textbf{Car}} & \multicolumn{1}{c}{\textbf{Chair}} & \multicolumn{1}{c}{\textbf{KITTI}} \\ \hline \hline
0    &      2.10                                 &      2.63                            &   3.02                                 &   0.132                              \\
0.25 &      \textbf{1.66}                                 &              \textbf{2.48 }                   &       \textbf{2.70}                             &          \textbf{0.095 }                         \\
0.5  &      2.31                                 &      3.00                            &       3.28                             &      0.121                              \\
0.75 &          2.59                             &              3.50                    &               3.78                     &              0.142                      \\
1    &      3.83                                 &  4.72                                &    4.95                                &         0.196                           \\ \hline
\end{tabular}} \\ \footnotesize{(a)} \\
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{c|llll}
\multirow{3}{*}{
\parbox{1.5cm}{\centering \textbf{Number of Regions Removed}}} & & & & \\  & \multicolumn{1}{c}{\textbf{Airplane}} & \multicolumn{1}{c}{\textbf{Car}} & \multicolumn{1}{c}{\textbf{Chair}} & \multicolumn{1}{c}{\textbf{KITTI}} \\
  & & & & \\ \hline \hline
0                      &    \textbf{1.66}                                   &        \textbf{2.48}                          &    \textbf{2.70}                                &      \textbf{0.095}                              \\
\hline
1                     &     1.67                                  &               2.50                   &          2.73                          &   0.097                                 \\
2                      &    1.76                                   &            2.60                      &         2.79                           &     0.100                               \\
3                      &    1.89                                   &             2.67                     &         2.95                           &       0.102                             \\
\hline
\end{tabular}} \\
 \footnotesize{(b)} \\
\end{tabular}
\caption{(a). Performance analysis on different values of hyperparameter $\beta$ used in Equation~\ref{equ:cd_global_loss}, (b). Chamfer Distance on Shapenet and KITTI with varying number of removed regions.}
\label{table:beta_table_old}
% \end{table}
\end{wraptable}

==> tables/emd_shapenet.tex <==
\begin{table}[h]
\centering
\begin{tabular} {l|ccc}
\textbf{Training Method}    & \textbf{Airplane} & \textbf{Car} & \textbf{Chair} \\ \hline \hline
\multicolumn{1}{l|}{DPC \cite{insafutdinov2018unsupervised}} & 0.146 & 0.160 & 0.194 \\
\multicolumn{1}{l|}{PointPnCNet (Ours)} & \textbf{0.108}  &  \textbf{0.120} &  \textbf{0.140} \\ \hline
\end{tabular}
\caption{Earth Mover Distance (EMD) results on Airplane, Cars, and Chairs categories of the Shapenet dataset. A lower EMD is better.}
\label{table:emd_shapenet}
% \vspace{-1em}
\end{table}



==> tables/kitti_main.tex <==
\begin{table}[h]
\small
\centering
\setlength{\tabcolsep}{1.5pt}
\begin{tabular} {l|ccc}
\textbf{Method} & \textbf{CD} & \textbf{Precision} & \textbf{Coverage} \\
\hline
\hline
\multicolumn{1}{l|}{Gu~\etal~\cite{gu2020weakly}} & 0.194 & 0.087 & 0.107 \\
\multicolumn{1}{l|}{Densified Input} & 0.130  & \textbf{0.025}  & 0.105   \\
\hline
\multicolumn{1}{l|}{PointPnCNet (Ours)} & \textbf{0.095}  &  0.045 &  \textbf{0.050} \\ \hline
\end{tabular}
\caption{Quantitative results on the Semantic KITTI dataset}
\vspace{-1em}
\label{table:kitti_main_results}
\end{table}

==> tables/kitti_metric.tex <==
\begin{table}[h]
\centering
\begin{tabular}{c|ll}
\textbf{Training Method} & \multicolumn{1}{c}{\textbf{F-score@1\%} $\uparrow$ } & \multicolumn{1}{c}{\textbf{EMD} $\downarrow$} \\ \hline \hline
 \multicolumn{1}{l|}{PointPnCNet (Ours)}       &    \textbf{0.67}                                      &                         \textbf{0.45}      \\ 
 \multicolumn{1}{l|}{Ours~w/o inpainting}           &            0.44                              &                 0.62                 \\
\hline  
\end{tabular}
\caption{F-Score@1\% and Earth Mover Distance (EMD) results on the Semantic KITTI dataset. We evaluate these metrics on our method vs our ablation of without inpainting.}
\label{table:kitti_metrics}
% \vspace{-1em}
\end{table}

==> tables/shapenet_pose_noise.tex <==
% \begin{table}[]
% \begin{tabular}{p{0.01\textwidth}p{0.08\textwidth}p{0.09\textwidth}|p{0.03\textwidth}p{0.03\textwidth}p{0.03\textwidth}}
% \textbf{Training Method} & \textbf{Rotation Noise (R)} & \textbf{Translation Noise (T)} & \multicolumn{1}{c}{\textbf{Airplane}} & \multicolumn{1}{c}{\textbf{Car}} & \multicolumn{1}{c}{\textbf{Chair}} \\ \hline \hline
% \multicolumn{1}{l}{Gu~\etal~\cite{gu2020weakly}} & 0 & 0 & \multicolumn{1}{c}{1.95} & \multicolumn{1}{c}{2.68} & \multicolumn{1}{c}{3.33} \\
% \hline
%  & $5^{\circ}$         & 0.01                 &    \multicolumn{1}{c}{1.89}                                   &    \multicolumn{1}{c}{2.51}                              &          \multicolumn{1}{c}{2.88}                          \\
% Ours & $10^{\circ}$         & 0.05                &          \multicolumn{1}{c}{1.90}                             &      \multicolumn{1}{c}{2.51}                            &  \multicolumn{1}{c}{2.93}                                  \\
%  & $15^{\circ}$        & 0.10                &        \multicolumn{1}{c}{1.94}                               &       \multicolumn{1}{c}{2.54}                           &    \multicolumn{1}{c}{2.98}                               
% \end{tabular}
% \end{table}


\begin{table}[]
\centering
\begin{tabular}{p{0.07\textwidth}|p{0.06\textwidth}p{0.09\textwidth}|p{0.06\textwidth}p{0.03\textwidth}p{0.03\textwidth}}
                         & \multicolumn{2}{c|}{Noise}                       &                   &              &                \\
\textbf{Training Method} & \textbf{Rotation (R)} & \textbf{Translation (T)} & \textbf{Airplane} & \textbf{Car} & \textbf{Chair} \\ \hline \hline
Gu et al                 & 0                     & 0                        & 1.95              & 2.68         & 3.33           \\ \hline
\multirow{3}{*}{Ours}    & 5                     & 0.01                     & 1.89              & 2.51         & 2.88           \\
                         & 10                    & 0.05                     & 1.90              & 2.51         & 2.93           \\
                         & 15                    & 0.1                      & 1.94              & 2.54         & 2.98  \\ \hline        
\end{tabular}
\caption{Chamfer Distance on the ShapeNet dataset for Airplane, Cars, and Chairs categories. We add a sampled noise to the predicted canonical pose for every partial point cloud. Rotation Noise depicts the noise sampled from [-R, R] degrees and translation noise sampled from [-T, T]. Translation is the  percent of object diameter. All results are multiplied by a factor of 100, following from Gu~\etal~\cite{gu2020weakly}.}
\label{table:shapenet_pose_noise}
\end{table}

